Crystalline Material Discovery in the Era of Artificial Intelligence

Crystalline materials, with symmetrical and periodic structures, exhibit a wide spectrum of properties and have been widely used in numerous applications across electronics, energy, and beyond. For crystalline materials discovery, traditional experimental and computational approaches are time-consuming and expensive. In these years, thanks to the explosive amount of crystalline materials data, great interest has been given to data-driven materials discovery. Particularly, recent advancements have exploited the expressive representation ability of deep learning to model the highly complex atomic systems within crystalline materials, opening up new avenues for fast and accurate materials discovery. These works typically focus on four types of tasks, including physicochemical property prediction, crystalline material synthesis, aiding characterization, and accelerating theoretical computations. Despite the remarkable progress, there is still a lack of systematic investigation to summarize their distinctions and limitations. To fill this gap, we systematically investigated the progress made in recent years. We first introduce several data representations of the crystalline materials. Based on the representations, we summarize various fundamental deep learning models and their tailored usages in various material discovery tasks. Finally, we highlight the remaining challenges and propose future directions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> ____________.tex <==
% \PassOptionsToPackage{table}{xcolor}
% \documentclass[fleqn,10pt]{wlscirep}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{multirow}
% \usepackage{tcolorbox}
% \usepackage[table]{xcolor}
% \tcbuselibrary{breakable}
% \usepackage{booktabs}
% \usepackage[table]{xcolor}
% \usepackage{graphicx,epstopdf}
% \usepackage{amsmath,amsthm,amssymb,amsfonts}
% \usepackage{tabularx,pdfcomment}
% \usepackage{graphicx,color,multirow,amsmath}
% \usepackage{cite}
% \usepackage{makecell}
% \usepackage{hyperref}
% \usepackage{comment}
% % \usepackage{xcolor}
% \usepackage{subfigure}
% \usepackage{hyperref}
% \usepackage{url}
% \usepackage{cases}
% \usepackage{bbm}
% \usepackage{bm}
% \usepackage{url}
% \usepackage{algpseudocode}
% \usepackage{algorithmicx}
% \usepackage{algorithm}
% \usepackage{graphicx} 

\newcommand{\wanyu}[1]{{\textcolor{blue}{\bfseries[wanyu says: #1]}}}
\newcommand{\zhong}[1]{{\textcolor{blue}{\bfseries[zz says: #1]}}}

\title{Crystalline Material Discovery in the Age of Artificial Intelligence}




\author[1]{Zhenzhong Wang}
\author[1]{Haowei Hua}
\author[1,2,*]{Wanyu Lin}
\author[3]{Ming Yang}
\author[2]{Kay Chen Tan}
\affil[1]{The Hong Kong Polytechnic University, Department of Computing}
\affil[2]{The Hong Kong Polytechnic University, Department of Data Science and Artificial Intelligence}
\affil[3]{The Hong Kong Polytechnic University, Department of Applied Physics}

% \affil[*]{e-mail: name.surname@email.edu}
%synthesis, crystal structure study, physicochemical properties

\begin{abstract}
Crystalline materials, exhibiting symmetrical and periodic structures, have a plethora of properties and have been widely used in various domains, such as sustainable development. To discover crystalline materials, traditional experimental and computational approaches are often time-consuming and expensive. In these years, thanks to the explosive amount of crystalline materials data, a great interest has been given to data-driven materials discovery. Particularly, the recent advancements exploit the expressive representation ability of deep learning to model the highly complex atomic systems within the crystalline materials, opening up new avenues for fast and accurate materials discovery. These works typically focus on three types of tasks, including physicochemical property prediction, crystalline material synthesis, aiding characterization, and force field development; these tasks are essential for scientific research and development in crystalline materials science. Despite the remarkable progress, there is still a lack of systematic research to summarize their correlations, distinctions, and limitations. To fill this gap, we first introduce several data representations of the crystalline materials. Based on the representations, we summarize various fundamental deep learning models and their tailored usages in material discovery tasks. We also point out the remaining challenges and propose several future directions. The main goal of this review is to offer comprehensive and valuable insights and foster progress in the intersection of artificial intelligence and material science. We have organized the surveyed work and benchmarking, and the corresponding sources can be accessed by the link xxx.


%property prediction, material generation, and force field development, which are essential for uncovering structure-property relationships. 
\end{abstract}
\begin{document}

\flushbottom
\maketitle

\thispagestyle{empty}


\section{Introduction}

%background, application, impact

Crystalline materials have been a cornerstone of materials science and engineering for centuries, with their unique properties and structures enabling a wide range of applications in fields such as electronics, sustainable energy, etc~\cite{gomes2021computational,ocp1111dataset,wang2024comprehensive,kuznetsov2010functional}. The term "crystalline" refers to the periodic arrangement of atoms, known as a crystal lattice. Within the crystal lattice, the atoms are structured by meticulously arranged symmetrical structures, fostering uniform atomic interactions. This long-range order characterized by periodicity and the short-range order featured by symmetry give rise to their stability~\cite{vainshtein2013fundamentals,luo2024towardssymmetry,xie2021crystal}. The distinctive structures of symmetry and periodicity also cultivate a rich tapestry of physical and chemical properties, enabling the versatility of crystalline materials. 


% Crystalline materials stand as pivotal keystones within numerous scientific and technological domains, prominently driving sustainable development initiatives like clean energy, carbon capture, and hydrogen storage~\cite{gomes2021computational,ocp1111dataset,wang2024comprehensive,kuznetsov2010functional}. Their stability owes much to meticulously arranged symmetrical structures and periodic atomic arrangement, fostering uniform atomic interactions~\cite{vainshtein2013fundamentals,luo2024towardssymmetry,xie2021crystal}.


% Crystalline materials, a branch of solid-state materials, possess symmetrical structures and periodic atom arrangements, contributing to uniform atomic interactions and their structure stability~\cite{vainshtein2013fundamentals,luo2024towardssymmetry,xie2021crystal}. The diverse crystal structures give rise to a wide range of properties, making crystalline materials functional for various applications, 

% including semiconductors, catalysts, alloys, etc~\cite{xiao2023invertible,ocp1111dataset,kozak2015single}.


%domain problems
Despite their widespread applications, crystalline materials are still not comprehensively understood, because their properties and structures are often complex and condition-dependent. The development of new crystalline materials with desired properties requires a deep understanding of structure-property relationships behind the materials~\cite{van2008complete,vu2023towards,liu2022experimental}. To uncover the structure-property relationships, hitherto, material science has gone through four paradigms~\cite{pyzer2022accelerating}. Before the 17th century, material science primarily relied on empirical and observational methods. In the 17th century, the advent of calculus initiated the second scientific revolution, a transition to theoretical science, characterized by mathematical equations of natural phenomena. The invention of computers in the 20th century created the third paradigm, the computational science paradigm, enabling larger and more complex theoretical equations to become solvable. Through computational simulations, e.g., density functional theory (DFT), new materials can be tested and evaluated. However, due to the vast number of possible combinations of elements, structures, and compositions, using these simulations to explore the structure-property relationships is of high computational cost and highly depends on the trial-and-error approaches~\cite{pyzer2022accelerating,lan2023adsorbml,xie2021crystal}. 

% In the past decade, the emergence of huge volumes of data has brought. With the vast amounts of data, 


% Among the data-driven methods, deep learning is attracting increasing attention due to its exceptional capacity for representation learning, showcasing remarkable accuracy and efficiency in crystalline materials. 

% The above three paradigms . Although expert knowledge is very useful in promoting physical understanding and generating new scientific hypotheses, traditional expert knowledge methods have significant limitations in terms of efficiency.

%machine learning/ AI /deep learning
In recent years, the fourth paradigm --- Artificial Intelligence (AI)-driven materials science~\cite{choudhary2020joint,himanen2019data,ocp1111dataset}, provides a new avenue for material discovery. Especially, the development of machine learning and deep learning techniques has revolutionized the field of materials science, enabling the rapid discovery of new materials. One of the key drivers of the advancements is the availability of large datasets from experiments and simulations~\cite{chanussot2021open,tran2023open}. For example, the Open Catalyst Project (OCP) has made available a vast dataset of crystal structures, consisting of 1.3 million molecular relaxations with results from over 260 million DFT calculations~\cite{zitnick2020introduction}. The tremendous data have provided a rich source of information for deep learning models to learn from, enabling them to automatically extract features to uncover complex patterns and relationships between material properties and structures, which has proven vital for characterizing crystalline materials. 


% In particular, the advancements of deep learning-driven crystalline material discovery have mainly benefited from the tremendous data from experiments or simulations~\cite{chanussot2021open,tran2023open}. 


Currently, deep learning-driven crystalline material discovery mainly offers a fresh perspective on property prediction, material generation, aiding characterization, and accelerating theoretical computations. Property prediction is a fundamental task in deep learning-driven materials science, where the goal is to predict the properties of a material based on its crystal structure. These models typically take the crystal structure and labeled property as input and output the predicted properties~\cite{xie2018crystal,schutt2018schnet,chen2019graph,zeni2023mattergen,cao2024space}. Material generation is the task of generating new crystal structures with specific properties. This task is particularly challenging, as it requires the model to generate a structure that is both stable and has the desired properties~\cite{xie2021crystal,zeni2023mattergen,cao2024space}. 
Aiding characterization is to use deep learning models to aid the quantitative or qualitative analysis of experimental observations and measurements, including assisting in the determination of crystal structure, identifying structural transition from X-ray, and inferring crystal symmetry from electron diffraction~\cite{ziletti2018insightful,yang2021deep,choudhary2022recent,el2019raman,lee2020deep}. Accelerating theoretical computations enables intractable simulations by reducing the computational cost for systems with increased lengths and timescales and providing potentials and functionals for complex interactions~\cite{behler2007generalized,chen2022universal,bartok2010gaussian,batzner20223}.

%  These models have been used to
% aid or even replace physical simulations or measurements under certain
% circumstances


% aid in the characterization of materials. This task is particularly important, as it enables researchers to quickly and accurately determine the properties of a material without the need for expensive and time-consuming experiments or simulations.


% The use of machine learning, especially deep learning, showcases high accuracy and efficiency in approximating computational simulations.



% can facilitate solutions for both the forward and inverse problem in photonics. We will examine how trained neural networks can function as high speed surrogate Maxwell solvers and how they can be configured to serve as high performance device optimizers. We note that there have been a number of recent reviews on machine learning and photonics20–22 that cover complementary topics to this Review, including reinforcement learning21, 23–25 and the application of photonics hardware to machine learning computation20,26. This Review is unique in that it serves as both a tutorial introducing basic machine learning concepts and a comprehensive guide for current state-of-the-art research developments. Additionally, it covers electromagnetic technologies spanning microwave to optical frequencies, providing a broader conceptual overview of the topic.

% De facto data format for recording these crystalline materials is Crystallographic Information File (CIFs). CIFs describe geometric information and non-geometric information about a crystal structure as text. The information includes atomic coordinates, coordinate types, atomic types, chemical elements, lattice parameters, symmetry information, etc~\cite{hall1991crystallographic}. The comprehensive information contained enables the CIFs to be invertible to the represented crystalline materials. In addition, in view of the string-based molecular representations, e.g., simplified molecular input line entry systems (SMILES)~\cite{weininger1988smiles}, an invertible string-based crystal representation, called simplified line-input crystal-encoding system (SLICES), is suggested to guarantee invertibility and invariances. Moreover, spectra-based crystal representations using electromagnetic radiation~\cite{chen2021direct,park2017classification} and image-based crystal representations using microscopy techniques~\cite{azimi2018advanced,modarres2017neural} are also widely used to analyze the composition, structure, and characteristics of crystalline materials.


% With the explosive and diverse crystalline material data, data-driven materials science has made noteworthy advancements in gaining insights into the structure-property relationships, such as property prediction, material generation, and force field development~\cite{pyzer2022accelerating,xie2018crystal,schutt2018schnet,chen2019graph,behler2007generalized,chen2022universal,bartok2010gaussian,batzner20223,zeni2023mattergen}. Property prediction aims to accurately determine or estimate the physical, chemical, or mechanical properties of materials based on their composition, structure, or other relevant characteristics~\cite{xie2018crystal,schutt2018schnet,chen2019graph,zeni2023mattergen,cao2024space}. One of the representative works is crystal graph convolutional neural networks (CGCNN)~\cite{xie2018crystal}. This work leverages geometric graphs as input and encodes both atomic information and bonding interactions to model the local environment of each atom. Material generation contributes to the optimization and design of novel materials with specific properties~\cite{xie2021crystal,zeni2023mattergen,cao2024space}. For example, Crystal Diffusion Variational Autoencoder (CDVAE)~\cite{xie2021crystal} was proposed by considering periodicity to explore the generation of stable materials in a diffusion process. Force field development is to establish force field models for molecular dynamics simulations~\cite{behler2007generalized,chen2022universal,bartok2010gaussian,batzner20223}. These models include potential energy functions and parameters that describe the interactions between atoms to simulate the structure, thermal properties, and mechanical properties of crystals. The representative one, M3GNet, utilizes a many-body computation module to calculate the three-body and many-body interaction atom indices, and the associated angle, showcasing the potential to learn the interatomic potential of various materials across the periodic table~\cite{chen2022universal}. These deep learning-driven works mainly leverage physical knowledge/constraints, such as symmetry and periodicity, into the deep learning models, such as geometric neural networks, generative models, and convolutional neural networks, to accurately model the complex atomic systems.




% Based on the explosive and various crystalline material data, machine learning in crystalline materials aims to assist researchers in trying to understand the structure-property relationships, which generally involve structure analysis, structure discovery, and property prediction. The goal of structure analysis in material science is to 1) gain a detailed understanding of crystallographic information, e.g., the arrangement and composition within a material, 2) understand phase transitions and transformations, and 3) assess microstructure. The structure analysis provides a basis for understanding the material's properties and performance. 


% Recent advancements in the field of crystalline materials have been made possible by the explosion of data from various applications, such as catalyst design and gas separation. One notable initiative in this regard is the Open Catalyst Project (OCP), which seeks to expedite the discovery of novel catalysts for renewable energy applications. The project boasts an extensive dataset comprising approximately 1.3 million crystalline materials, obtained through a staggering 260 million density functional theory (DFT) calculations. Researchers also employed diverse data representations for crystal materials, these representations encompass atomic representation, string representation, descriptor representation, spectral representation, and image representation. Each of these representations possesses distinct characteristics in terms of granularity, storage efficiency, and acquisition cost. By utilizing these varied representations, researchers can gain valuable insights into the properties and behavior of crystalline materials, facilitating the development of advanced crystalline material discovery.

% Based on the explosive and various crystalline material data, machine learning in crystalline materials aims to assist researchers in trying to understand the structure-property relationships, which generally involve structure analysis, structure discovery, and property prediction. The goal of structure analysis in material science is to 1) gain a detailed understanding of crystallographic information, e.g., the arrangement and composition within a material, 2) understand phase transitions and transformations, and 3) assess microstructure. The structure analysis provides a basis for understanding the material's properties and performance. Structure discovery contributes to the prediction, optimization, and design of novel materials with specific properties. Property prediction is to accurately determine or estimate the physical, chemical, or mechanical properties of materials based on their composition, structure, or other relevant characteristics.

In this review, we will discuss how deep neural networks can facilitate crystalline material discovery tasks. We will investigate how deep neural networks leverage different data representations and incorporate physical knowledge/constraints to model the complex atomic systems within crystalline materials, and how deep neural networks function as accurate and efficient surrogate solvers to approximate expensive computational simulations. 
We note that there have been a number of recent reviews on deep learning and crystalline materials that cover complementary topics to this review~\cite{choudhary2022recent,han2022geometrically}. This review is unique in that it serves as both a tutorial introducing basic crystalline materials concepts, recent cutting-edge models, and comprehensive guide for current state-of-the-art research developments, distinctions, and limitations, which provide a broader conceptual overview of this intersection of disciplines of AI and crystalline materials.

% The use of machine learning, especially deep learning, showcases high accuracy and efficiency in 
% Although deep learning models have been increasingly applied in the field of crystalline material research, there is still a need for a systematic summary of this fast-growing field. 

% While reviews have covered deep learning-driven material discovery~\cite{choudhary2022recent,han2022geometrically}, they omitted coverage of recently cutting-edge models, such as geometric neural networks, large language models, diffusion models, in material discovery or did not focus on clarifying concepts in the field of crystalline materials.
% To the best of our knowledge, this is the first comprehensive review of crystalline materials, with a specific emphasis on the recent advances in deep learning models and their correlations, distinctions, and progress. The primary objective of this review is to provide valuable insights to researchers working in the domains of crystalline materials and deep learning, aiding them in the development of more effective and efficient approaches tailored to crystalline materials. By offering a comprehensive overview and analysis of the current state of deep learning models to crystalline materials, this review aims to contribute to the advancement of research and innovation in this intersection of disciplines.

 % We summarize these works by highlighting the used data representation, physical knowledge/constraints, characteristics, and shortcomings. 

An overview of this review’s organization is shown in FIG. \ref{fig:outline}. In the review, we provide illustrations of data representations that have been used in crystalline material research. The data representations involve geometric graphs, text representation, images, and spectra. With the different data representations, foundation models such as geometric neural networks, language models, and convolutional neural networks and their design principles are introduced. Then, we mainly focus on the recent works on property prediction, material generation, aiding characterization, and accelerating theoretical computations. In addition, we provide some of the commonly used datasets, benchmarks, and software used for data-driven crystalline material discovery. It is worth noting that while deep learning has facilitated the development of crystalline material discovery, there are many challenges and issues that need to be addressed to unleash the potential of deep learning for crystalline materials further, such as explainability, humans in the loop, and generalizability. Therefore, we also highlight these challenges and provide insights in this domain.

\begin{figure*}[htbp] 
  \centering   
  \includegraphics[width=16.9cm]{fig/outline.pdf}
  \caption{An overview of this review’s organization.}
  \label{fig:outline}
\end{figure*} 
% Its notable strength is often accompanied by a trade-off in terms of explainability. The limited interpretability of deep learning models has hindered their practicality in materials science tasks. Furthermore, the high cost associated with data collection, coupled with low data availability and low data quality, poses challenges to the generalizability of deep learning models in this field. Additionally, the often absence of explicit incorporation of physical information within deep learning models poses a barrier to accurately describing atomic systems, thereby leaving room for improvement in model accuracy. Consequently, 



% The rest of the paper is organized as follows: Section II gives a foundation of data representations. The relevant base neural networks to these data representations are briefly presented in Section III. Section IV discusses the deep learning-assisted research tasks in crystalline materials. Section V summarizes the benchmark and software platform,
% Section VI discusses the insights and future outlooks in the research of crystalline materials. Lastly, Section VII concludes this review and suggests future directions.

\begin{figure}[h] 
  \centering   
\includegraphics[width=16.7cm]{fig/datamodel.pdf} 
  \caption{Overview of deep learning for crystalline materials. \textbf{a|} Crystalline materials are described by geometric graphs. Typically, geometric neural networks are used to extract node, edge, and directional information from the geometric graphs by message passing mechanism. The extracted embedding serves for various downstream tasks. \textbf{b|} For string data, such as CIF and SLICES, language models are generally used to handle the sequence data. Language models can be fine-tuned for various downstream tasks. \textbf{c|} The atomic image and spectra data of crystalline materials are processed using convolutional neural networks, and convolutional kernels transform these data into feature map representations. \textbf{d|} The above fundamental models serve as surrogates for various material discovery tasks, including physicochemical property prediction, crystalline material synthesis, aiding characterization, and force field development.
  }
  \label{fig:cif}
\end{figure} 


\section{Data Representations Describing Crystalline Materials}


%Crystalline materials are structured as a periodic arrangement of atoms in 3D space, with the repeating unit known as the unit cell. This unit cell comprises a collection of atoms characterized by their types and coordinates. The shape and dimensions of the unit cell are described by the lattice parameters, which encompass the lengths of the unit cell edges and their respective angles (often depicted using vectors). By employing translational operations to replicate the unit cell in space, the entire crystal structure can be constructed. The above geometric information and non-geometric information of crystalline materials are detailed in CIFs. In addition, by deciphering the CIFs, geometric graphs of crystalline materials can also be well modeled. Apart from CIFs, researchers also employ electronic imaging methods and electromagnetic radiation to obtain atomic images and spectra data to characterize the materials. This section introduces the above four types of data representation for crystalline materials: text, geometric graphs, images, and spectra data.
Crystalline materials exhibit a highly ordered structure characterized by a periodic arrangement of atoms in 3D space. The fundamental repeating unit within this structure is known as the unit cell, which consists of a specific arrangement of atoms, each defined by their types and coordinates. The shape and dimensions of the unit cell are articulated by the lattice parameters, including the lengths of the unit cell edges and the angles between them, often represented through vectors. By applying translational operations to replicate the unit cell throughout space, the comprehensive crystal structure is constructed.
The above geometric and non-geometric information of crystalline materials is meticulously documented in Crystallographic Information Files (CIFs), which provide a comprehensive description of the crystal's atomic configuration and facilitate the modeling of geometric graphs of crystalline materials. In addition to CIFs, researchers employ advanced techniques such as electronic imaging methods and electromagnetic radiation to capture atomic images and spectra data, further characterizing the material.
This section introduces the above four types of data representation for crystalline materials: text, geometric graphs, images, and spectra data.

\subsection{String Representations}




% \zhong{talk about Crystallographic Information File first, then discuss invertible, invariant representation SLICES}

% In many fields, there are numerous cases where text is employed to represent data. For instance, the FASTA format is used for representing nucleotide or peptide sequences \cite{lipman1985rapid}.
% In seismic exploration, SEG-Y files are utilized to store seismic waveform data, sampling rates, recording times, and other pertinent information \cite{barry1975recommended}.



%CIFs are the de facto data format of crystalline materials~\cite{hall1991crystallographic}, which record comprehensive information about a crystal structure as text. As shown in FIG. \ref{fig:spectra}a, the CIF file records detailed information about atom type, atom coordinates, lattice parameters, space groups, and other structural characteristics in textual form. A number of studies directly use CIFs as the text input and employ language models for different downstream tasks\cite{gruver2024finetuned,cao2024space}. 
CIFs are the de facto standard for representing crystalline material data ~\cite{hall1991crystallographic}. This kind of data encapsulates comprehensive details about a crystal structure in text format, including atom types, atomic coordinates, lattice parameters, space groups, and other structural attributes,fig:spectra as illustrated in FIG. \ref{fig:spectra}a. Numerous studies leverage CIFs as text inputs, employing language models for various downstream tasks \cite{gruver2024finetuned, cao2024space}.



% \begin{figure}[h] 
%   \centering   
%   \includegraphics[width=6.0in]{fig/CIF-slice3.pdf} 
%   \caption{\textbf{Examples of CIF and SLICES.}
%   To illustrate the CIF and SLICES, we use the example of Li$_2$CoO$_2$ (ID: mp-755297, from the Materials Project~\cite{jain2013commentary}).  
%   \textbf{a $|$} The crystal structure of Li$_2$CoO$_2$.
%   \textbf{b $|$} The information contained in the CIF file of Li$_2$CoO$_2$.
%   \textbf{c $|$} SLICES string representation of Li$_2$CoO$_2$. 
%   }
%   \label{fig:cif}
% \end{figure} 



%Text-based representations, e.g., simplified molecular input line entry systems (SMILES~\cite{weininger1988smiles}), have stood out for simplicity and adaptability in molecule domains. The text-based representation can be viewed as a form of "chemical" language and thus is widely used to unleash the use of language models.







% in recent years, with increased application for machine learning, CIF format has become inadequate for certain specific requirements. For example, if models directly utilize CIF as a data input format, the direct recording of atomic fractional coordinates in CIF poses challenges in ensuring model invariance. Additionally, the overly redundant information in CIF format increases the difficulty for the model to process it.

\begin{comment}
\begin{figure*}[h] 
  \centering   
  \includegraphics[width=14cm]{fig/slice-example.pdf}
  \caption{\textbf{A schematic diagram of converting crystal structures to SLICES strings} (figure obtained from REF. \cite{chen2022universal}).}
  \label{fig:slice}
\end{figure*} 
\end{comment}


% Previous research in the molecular domain has provided insights into more suitable text representations of crystals for machine learning. Text-based simplified molecular representations, such as the Simplified Molecular Input Line Entry System (SMILES \cite{weininger1988smiles}), have stood out due to their simplicity and adaptability.
% This kind of text-based representation can be viewed as a form of "chemical" language and thus is widely used to unleash the use of language models.
% By viewing the text-based representation as a form of "chemical" language, language models have could offer higher throughput and accuracy for molecular property prediction~\cite{gong2024text,mokaya2023testing}.
% However, the design of string-based representations for crystalline materials is a long-standing challenge as the desirable representations should be invertible, invariant, periodicity-aware, and cover the majority of elements across the periodic table. 

% To address the issue, a string-based invertible crystal representation that guarantees invariances, a simplified line-input crystal-encoding system (SLICES) is proposed~\cite{xiao2023invertible}. 

However, directly utilizing CIFs as text poses challenges in ensuring invariance. In molecule domains, several invertible and invariant representations, such as simplified molecular-input line-entry (SMILES)~\cite{weininger1988smiles} and self-referencing embedded strings (SELFIES)~\cite{krenn2020self} have stood out for simplicity and adaptability. Toward invertible, invariant, periodicity-aware text-based representation for crystalline materials, Xiao \textit{et. al.,} proposed simplified line-input crystal-encoding system (SLICES)~\cite{xiao2023invertible}.
In SLICES, the quotient graph~\cite{chung1984nomenclature} serves as an intermediary to translate between crystal structures and SLICES strings. The quotient graph indicates how atoms in a unit cell are connected to atoms in adjacent unit cells. For instance, as depicted in FIG. \ref{fig:spectra}b, the edge $e_4$ is labeled ‘0 0 1’ in the quotient graph, indicating that $e_4$ connects node C$_0$ to the copy of C$_1$ shifted one unit along the $c$ axis. SLICES strings convert the quotient graph into three components: atomic symbols, node indices, and edge labels.
A SLICES string begins with the atomic symbols of the unit cell, encoding the chemical composition of the crystal structure. Edges are explicitly represented explicitly in the form $uvxyz$, where $u$ and $v$ are node indices, and $xyz$ denotes the location of the unit cell to connect to. Specifically, to represent the quotient graph in FIG. \ref{fig:spectra}b, the SLICES string begins with atom symbols C$_0$ and C$_1$ of node indices $0$ and $1$, respectively. Following the atom symbols, the edges $e_1\ldots e_4$ of the form $uvxyz$ in the quotient graph are appended. For instance, $e_4$ is represented as `01oo+'. Here, $01$ denotes the atomic indices corresponding to the positions in the atomic symbols of the SLICES string (i.e. C$_0$ and C$_1$). The sequence `oo+' represents the label ‘0 0 1’ from the labeled quotient. In SLICES, graph theory and force field approaches are used to reconstruct the corresponding crystal structure from the SLICES strings to ensure the invariances and invertibility.


% After obtaining the SLICES string representation,  are used to reconstruct the corresponding crystal structure. For instance, Fig. \ref{fig:cif} (c) presents a SLICES string of Li$_2$CoO$_2$.
% As shown in Fig. \ref{fig:slice}, SLICES strings first encode all atoms in the unit cell by sequentially arranging them as atomic symbols. Then, the connections between the atoms are encoded by their node indices and the edges connecting them. 



%A SLICES string always begins with symbols of atoms in the unit cell (Fig. \ref{fig:slice}), encoding the chemical composition of the corresponding crystal structure. In SLICES, edges are represented explicitly in the form $u,v,x,y,z$, where $u,v$ are node indices and $x,y,z$ denotes the location of the unit cell to connect to. In essence, edge labels specify the translation vectors needed to connect unit cells. The string representation is constructed by encoding the atomic symbols, node indices, and the aforementioned edge labels. To ensure the invertibility and invariances, SLICES uses graph theory techniques, optimization based on geometry predicted with geometry frequency noncovalent force field, and graph deep learning interatomic potential~\cite{chen2022universal} to accurately rebuild input crystal structures.


\subsection{Geometric Graph Representations}

% Crystalline materials can be naturally represented in the Euclidean space. The quantities in the Euclidean space, e.g., the positions of the atoms, depict the geometry of the materials. 

%With the geometry of crystalline materials recorded in CIFs, geometric graphs of crystalline materials in Euclidean space can be well modeled. Here, we introduce two commonly utilized coordinate systems—namely, the Cartesian coordinate system and the fractional coordinate system—to represent the geometric layout of crystalline materials.
With the geometric details of crystalline materials meticulously recorded in CIFs, it becomes feasible to effectively model geometric graphs of these materials within Euclidean space. In this context, we introduce two widely utilized coordinate systems—namely, the Cartesian coordinate system and the fractional coordinate system—as fundamental tools for representing the geometric configuration of crystalline materials.

% Crystalline materials can be represented as the periodic arrangement of atoms in the 3D space. The repeating unit is called unit cell. The unit cell contains a set of atoms with their atom types and coordinates. The geometric shape and size of the unit cell are determined by the lattice parameters. These parameters include the lengths of the unit cell edges and their angles (which can also be represented using vectors). By repeating the unit cell through translational operations in space, the entire crystal can be formed. In this part, we introduce two coordinate systems, i.e., the Cartesian coordinate system and the fractional coordinate system, which are widely used to represent the geometric graph of crystalline materials. 

% To avoid describing all the atoms within a crystal, a set of non-repeating fundamental atoms, known as the unit cell~\footnote{\hhw{The repeating unit in crystals is called unit cell. The unit cell contains a set of atoms with their atom types and coordinates. The geometric shape and size of the unit cell are determined by the lattice parameters. These parameters include the lengths of the unit cell edges and their angles (which can also be represented using vectors). By repeating the unit cell through translational operations in space, the entire crystal can be formed.}}, along with their repetitive arrangement, is often used to describe the crystal. In this section, we introduce the geometric representation of crystals based on two coordinate systems: the Cartesian coordinate system and the fractional coordinate system.}



% \zhong{some important concepts are not well introduced, for example, unit cell? lattice parameters? please refer to \cite{NEURIPS2023_38b787fc,xie2021crystal} to improve this part.
% \textcolor{cyan}{response:Related concepts have been added below.}}



%The crystal structure can be represented as the periodic repetition of a unit cell in three-dimensional (3D) Euclidean space, where the unit cell encompasses the smallest repeatable structure of the given crystal. By knowing the coordinates of all atoms within the unit cell and the periodic repetition pattern of the unit cell, one can determine the infinite atomic point cloud data throughout the entire crystal material.


 

%In the field of AI for crystal materials, current research utilizes multiple matrix data to describe crystal structures \cite{taniai2024crystalformer,lin2023efficient,wang2024conformal}.


% \begin{tcolorbox} [boxrule=.2mm,arc = 0mm, outer arc = 0mm,left=0.2mm,right=0.2mm,top=0.3mm,bottom=0.3mm,colback = white]
% \noindent \textbf{Box 1 | Title.}
% Word count up to 600 words. Boxes can include small illustrations. Any figures included in boxes should be described in full in the box text — a separate figure caption is not used. Boxes can also contain small tables. Boxes should be included in the manuscript Word document.  Please include them at the end of the article (i.e. the present location in this template) rather than at the position you’d like the box to be in within the main text.  However, please add a call out in the main text for ‘Box 1’.
% \end{tcolorbox}

\textbf{Cartesian Coordinate System}. A crystalline material can be formally  represented as $\mathbf{M}=(\mathbf{A},\mathbf{X},\mathbf{L})$, where $\mathbf{A}=[\boldsymbol{a}_1,\boldsymbol{a}_2,\cdots,\boldsymbol{a}_n]^T\in\mathbb{R}^{n\times d_a}$ denotes the atom feature matrix for $n$ atoms within a unit cell, with $\boldsymbol{a}_{i}\in\mathbb{R}^{d_{a}}$ representing the $d_{a}$-dimensional feature vector of an individual atom, such as the atomic type. The matrix $\mathbf{X}=[\boldsymbol{x}_{1},\boldsymbol{x}_{2},\cdots,\boldsymbol{x}_{n}]^{T}\in\mathbb{R}^{n\times3}$ represents the 3D Cartesian coordinates of $n$ atoms within an unit cell, where $x_i\in\mathbb{R}^3$ specifies the Cartesian coordinates of each atom. %With $(\mathbf{A},\mathbf{X})$, the structure of a single unit cell is represented. 
Then, the repeating patterns of the unit cell can be described by 
the lattice matrix $\mathbf{L}=[\boldsymbol{l}_{1},\boldsymbol{l}_{2},\boldsymbol{l}_{3}]\in\mathbb{R}^{3\times3}$, where $\boldsymbol{l}_{1}$, $\boldsymbol{l}_{2}$, and $\boldsymbol{l}_{3}$ are a set of basis vectors in 3D Euclidean space. The unit cell repeats itself along these three basis vector directions to form a complete crystal. 
Finally, A complete crystal can be represented as $(\hat{\mathbf{A}}, \hat{\mathbf{X}})=\{(\hat{\boldsymbol{a}_{i}}, \hat{\boldsymbol{x}}_i)|\hat{\boldsymbol{x}}_i=\boldsymbol{x}_i+k_1\boldsymbol{l}_1+k_2\boldsymbol{l}_2+k_3\boldsymbol{l}_3, \hat{\boldsymbol{a}_{i}}=\boldsymbol{a}_{i},k_1,k_2,k_3\in\mathbb{Z},i\in\mathbb{Z},1\leq i\leq n\}$. Here, the integers $k_i$ and $l_i$ represents all possible atomic positions in the periodic lattice.


\begin{figure}[b!] 
  \centering   
  \includegraphics[width=6.3in]{fig/p4mm2.pdf}
  \caption{
  \textbf{Examples of the Wyckoff positions for the 2D plain group P4mm.}
  \textbf{a $|$} The Wyckoff positions of the P4mm space group (No.11).
  \textbf{b $|$} The schematic diagram for the Wyckoff positions of the P4mm space group. 
  }
  \label{fig:p4mm}
\end{figure} 


% \vspace{0.5cm}
% \textbf{Fractional Coordinate System} 
% \label{Wyckoff}
% \zhong{the difference between fractional and Cartesian? please refer to \cite{NEURIPS2023_38b787fc,cao2024space} to improve this part. please also mention the connection to Wyckoff positions\cite{cao2024space},\textcolor{cyan}{response:}}

% In certain studies involving crystal generation \cite{jiao2023crystaliclr,song2024diffusion}, A fractional coordinate representation method is commonly employed. This representation, where coordinate values are within a specific range, proves beneficial in these research endeavors, particularly in facilitating the generation of atomic positions.

\textbf{Fractional Coordinate System}. 
In contrast to directly defining the positions of atoms in a crystal using three standard orthogonal bases in the Cartesian coordinate system, the fractional coordinate employs $\mathbf{L}=[\boldsymbol{l}_{1},\boldsymbol{l}_{2},\boldsymbol{l}_{3}]\in\mathbb{R}^{3\times3}$ as the basis vectors for atomic positions. Here, the position of an atom can be represented by a fractional coordinate vector $\boldsymbol{f_{i}}=[f_{1},f_{2},f_{3}]^{T}\in[0,1)^{3}$. The corresponding Cartesian coordinate vector can be expressed as %$\boldsymbol{p}=\sum_{i=1}^{3}f_{i}\boldsymbol{l}_{i}$.
$\boldsymbol{x}_{i}=f_{i}\boldsymbol{l}_{i}$. Therefore, for a crystal $\mathbf{M}$, it can be represented as $\mathbf{M} = (\mathbf{A}, \mathbf{F}, \mathbf{L})$, where $\mathbf{F}=[\boldsymbol{f}_1,\cdots,\boldsymbol{f}_n]^{T}\in[0,1)^{n\times 3}$ represents the fractional coordinates of all the atoms in the unit cell.


The fractional coordinate system efficiently captures the relative positions of atoms within a unit cell, thereby allowing for convenient expression of equivalent positions in a crystal structure generated by symmetry transformations of the space group. Below, we briefly introduce the concept of space groups and the representation of equivalent positions using fractional coordinates.

Crystals inherently exhibit symmetric structures characterized by space groups, resulting from the combination of rotational and translational symmetry in space~\cite{jiao2024space, cao2024space}.  
Specifically,
given a transformation $g\in\mathrm{E}(3)$ (See Box 1), the transformation of the coordinate matrix $\mathbf{X}$ can be expressed as $g\cdot\mathbf{X}:=\mathbf{Q}\mathbf{X}+\boldsymbol{b}$, 
where $\mathbf{Q}\in\mathbb{R}^{3 \times 3}$ is an orthogonal matrix and $\boldsymbol{b}\in\mathbb{R}^{3}$ is a translation vector. A crystal $\mathbf{M}$ is recognized to be symmetric with respect to $g$ if $g\cdot\mathbf{M}=\mathbf{M}$. Specifically, there exists a permutation matrix $\mathbf{P}\in\{0,1\}^{n\times n}$ that maps each atom to its corresponding symmetric point, such that $\mathbf{A}=\mathbf{P}\mathbf{A},g\cdot\mathbf{X}=\mathbf{P}\mathbf{X}$.
The set of all possible symmetric transformations $g$ of $\mathbf{M}$ constitutes a space group.
Due to the periodicity of crystals, the set of all possible symmetric transformations $g$ is finite~\cite{jiao2024space}, and the total number of different space groups is also finite. Accordingly, space groups are classified into 230 types for 3D crystal structures~\cite{jiao2024space,hahn1983international}.
The finite space group also imposes strict constraints on specific positions of atoms within the crystal structure, known as Wyckoff positions.




Wyckoff positions describe a set of symmetric positions within the unit cell\cite{jiao2024space,cao2024space}. Wyckoff Positions include three elements: multiplicity, Wyckoff letter, and fractional coordinates. For instance, FIG. \ref{fig:p4mm}a shows the Wyckoff positions for the 2D plain group P4mm \cite{hahn1983international}.
These positions are labeled using Wyckoff letters from the alphabet. The multiplicity indicates the number of equivalent positions derived from the symmetry transformations of the space group. To preserve the symmetry of the space group, these positions must all be occupied by the same type of atom. In the associated fractional coordinate representation, $x$ and $y$ are fractional coordinates where $0\leq x\leq 0.5;0\leq y\leq 0.5;x\leq y$. FIG. \ref{fig:p4mm}b presents a schematic diagram of the Wyckoff positions, with equivalent positions marked by the same color.




% Since Wyckoff positions are defined within the unit cell, the same type of Wyckoff position in different crystals can be represented by uniform fractional coordinates.

% Space groups impose strict conditions on the specific positions of atoms within the crystal and the total number of atoms in each unit cell. Atoms will only occupy specific positions within the unit cell, known as Wyckoff positions (see \ref{Wyckoff})
% Space groups impose strict conditions on the specific positions of atoms within the crystal and the total number of atoms in each unit cell. Atoms will only occupy specific positions within the unit cell, known as Wyckoff positions (see \ref{Wyckoff}).

% \zhong{making the logic of the following paragraph clearer}

% Additionally, space groups can identify the crystal family to which the crystal belongs, thereby constraining the permissible values of the lattice parameters. Specifically, for a crystal $\mathbf{M}=(\mathbf{A},\mathbf{C},\mathbf{L})$, the lattice matrix $\mathbf{L}$ is invertible and it has the
% Polar Decomposition \cite{hall2013lie}:

% An invertible matrix $\mathbf{L}\in\mathbb{R}^{3\times3}$ can be uniquely decomposed into $\mathbf{L}=\mathbf{O}\exp(\mathbf{S})$, where $\mathbf{O}\in\mathbb{R}^{3\times3}$ is an orthogonal matrix, $\mathbf{S}\in\mathbb{R}^{3\times3}$ is a symmetric matrix and $\exp(\mathbf{S})=\sum_{n=0}^\infty\frac{\mathbf{S}^n}{n!}$ defines the exponential mapping of $\mathbf{S}$. The above proposition indicates that $\mathbf{L}$ can be uniquely represented by $\mathbf{S}$. This is because $\mathbf{O}$ can be equivalently transformed by $O(3)$, meaning that regardless of how the crystal structure is rotated in space, the $\mathbf{S}$ corresponding to $\mathbf{L}$ remains invariant.


% According to \cite{jiao2024space}, 6 bases of the space of symmetric matrices can be found, e.g.,
% \begin{equation*}
% \scalebox{0.8}{\begin{gathered}\mathbf{B}_1=\begin{pmatrix}0&1&0\\1&0&0\\0&0&0\end{pmatrix},\mathbf{B}_2=\begin{pmatrix}0&0&1\\0&0&0\\1&0&0\end{pmatrix},\mathbf{B}_3=\begin{pmatrix}0&0&0\\0&0&1\\0&1&0\end{pmatrix},\\\mathbf{B}_4=\begin{pmatrix}1&0&0\\0&-1&0\\0&0&0\end{pmatrix},\mathbf{B}_5=\begin{pmatrix}1&0&0\\0&1&0\\0&0&-2\end{pmatrix},\mathbf{B}_6=\begin{pmatrix}1&0&0\\0&1&0\\0&0&1\end{pmatrix}.\end{gathered}}
% \end{equation*}
% Each symmetric matrix can be expanded via the above symmetric bases as stated below \cite{jiao2024space}.



% $\forall\mathbf{S}\in\mathbb{R}^{3\times3},\mathbf{S}=\mathbf{S}^\top,\exists\boldsymbol{k}=(k_1,\cdots,k_6),s.t.\mathbf{S}=\sum_{i\mathbf{=}1}^6k_i\mathbf{B}_i$


% It is clear to find that $\mathbf{L}$ is determined by the values of $k_i$. Therefore, the constraints of the space group acting on $\mathbf{L}$ can be reflected by different combinations of the symmetric bases. Actually, the total 230 space groups are classified into 6 crystal families, determining the shape of $\mathbf{L}$, and the correspondence between the crystal families and the values of $k_i$ is given in the Table \ref{tab:crystal_families}.

%Space group symmetry imposes significant constraints on a crystal. At its core, the space group identifies the crystal system to which a crystal belongs, thereby limiting the permissible values for the lattice parameters that define the dimensions and angles of the crystal’s unit cell.

% \begin{table*}[htbp]
% \centering
% \caption{Constraints for different crystal families and their space groups.}
% \begin{tabular}{cccc}
% \toprule
% \textbf{Crystal Family} & \textbf{Space Group No.} & \textbf{Lattice Shape} & \textbf{Constraint of Symmetric Bases} \\
% \hline 
% Triclinic & 1$\sim$2 & No Constraint & No Constraint \\
% \hline
% Monoclinic & 3$\sim$15 & $\alpha = \gamma = 90^\circ$ & $k_1 = k_3 = 0$ \\
% \hline
% Orthorhombic & 16$\sim$74 & $\alpha = \beta = \gamma = 90^\circ$ & $k_1 = k_2 = k_3 = 0$ \\
% \hline
% Tetragonal & 75$\sim$142 & $\alpha = \beta = \gamma = 90^\circ$ & $k_1 = k_2 = k_3 = 0$ \\
% & & $\alpha = b$ & $k_4 = 0$ \\
% \hline
% Hexagonal & 143$\sim$194 & $\alpha = \beta = 90^\circ, \gamma = 120^\circ$ & $k_2 = k_3 = 0, k_1 = -\log(3)/4$ \\
% & & $\alpha = b$ & $k_4 = 0$ \\
% \hline
% Cubic & 195$\sim$230 & $\alpha = \beta = \gamma = 90^\circ$ & $k_1 = k_2 = k_3 = 0$ \\
% & & $a = b = c$ & $k_4 = k_5 = 0$ \\
% \bottomrule
% \end{tabular}
% \label{tab:crystal_families}
% \end{table*}










% \begin{table*}[htbp]
%   \centering
%   \caption{}%0≤x≤0.5;0≤y≤0.5;x≤y
%   \resizebox{\textwidth}{!}{%
%     \begin{tabular}{lll}
%     \toprule
%     Multiplicity & Wyckoff letter & Fractional coordinates  \\
%     \midrule
%     8 &g & (x,y), (x,-y), (-x,y), (-x,-y),(y,x), (y,-x), (-y,x), (-y,-x)  \\
%     4 &f & (x,x), (x,-x), (-x,x), (-x,-x)  \\
%     4 &e & (x,1/2), (-x,1/2), (1/2,x), (1/2,-x)  \\
%     4 &d & (x,0), (-x,0), (0,x), (0,-x) \\
%     2 &c & (1/2,0), (0,1/2) \\
%     1 &b & (1/2,1/2) \\
%     1 &a &  (0,0) \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:p4mm}%
% \end{table*}%


% \subsubsection{Descriptor}



% \subsubsection{Periodic Table Based Representation}
% To address the scalability issues of the model, researchers in \cite{yang2023scalable} developed a unified crystal representation that can represent any
% crystal structure (UniMat). 
% %As shown in Fig. \ref{fig:periodic_table_representation}, 
% UniMat represents crystals based on the rich prior knowledge of chemical properties from the periodic table, using a 4-dimensional material space $\mathcal{M}:=\mathbb{R}^{L\times H\times W\times C}$ to represent the atomic composition and spatial coordinates of crystal materials. Here, $H = 9$ and $W = 18$ correspond to the number of periods and groups in the periodic table, which can be used in combination to represent the types of atoms in a crystal.
% $L$ corresponds to the maximum number of atoms per element in the periodic 
% table, i.e the number of atoms per element in a crystal, and $C = 3$ corresponds to the coordinate of each atoms in a unit cell. 
% Authors of UniMat define a null coordinate using special values such as $(-1,-1,-1)$ to represent the absence of this atom.
%Despite the lack of explicit structural modeling, UniMat can generate high-fidelity crystals from larger and more complex chemical systems in generative method applications, outperforming previous methods \cite{yang2023scalable}.

% \begin{comment}
% \begin{figure}[h] 
%   \centering   
%   \includegraphics[width=3.3in]{fig/periodic_table_representation.pdf}
%   \caption{UniMat representation of crystal structures. Crystals are represented by the atom locations stored
% at the corresponding elements in the periodic table (and additional unit cell parameters if coordinates are fractional). For instance, the bottom right atom Na in the crystal is located at $(0.5,0,0)$, hence the periodic table has value $(0.5,0,0)$ at the Na entry. (figure obtained from \cite{yang2023scalable}).}
%   \label{fig:periodic_table_representation}
% \end{figure} 
% \end{comment}

\begin{comment}
\begin{figure}[h] 
  \centering   
  \includegraphics[width=6.3in]{fig/image-spectra.pdf} 
  \caption{
\textbf{Examples of data representations: images and spectra data.}
To illustrate the diffraction
image, X-ray diffraction spectra, and Raman spectra, we use the example of Fe$_2$O$_3$ (MP ID: mp-19770, from the Materials Project~\cite{jain2013commentary}. ROD ID: 1000001, from the Raman Open Database~\cite{el2019raman}).  
\textbf{a $|$} The crystal structure of Fe$_2$O$_3$.
\textbf{b $|$} The X-ray diffraction spectra of Fe$_2$O$_3$ (generated by Pymatgen~\url{https://pymatgen.org/}). 
\textbf{c $|$} The electron diffraction image of Fe$_2$O$_3$. 
\textbf{d $|$} The Raman spectra of Fe$_2$O$_3$. 
}
  
  \label{fig:spectra}
\end{figure} 
\end{comment}

\begin{figure}[t!] 
  \centering   
  \includegraphics[width=16.7cm]{fig/datarep.pdf} 
  \caption{
\textbf{Examples of data representations: texts, images and spectra data.}
%To illustrate images and spectra data representations, we use the example of BaTiO$_3$ (MP ID: mp-5986, from the Materials Project~\cite{jain2013commentary}.).  
\textbf{a $|$} The CIF of BaTiO$_3$ (MP ID: mp-5986, from the Materials Project~\cite{jain2013commentary}.).
\textbf{b $|$} The illustration of SLICES string conversion process. 
\textbf{c $|$} The STEM image and the X-ray diffraction spectra data. 
%\textbf{c $|$} The electron diffraction image of BaTiO$_3$ and the X-ray diffraction spectra of BaTiO$_3$ (generated by Pymatgen~\url{https://pymatgen.org/}). ~\cite{ge2022atomic}
}
  \label{fig:spectra}
\end{figure} 


\subsection{Image Representations}

% \zhong{please briefly introduce this by referring to \cite{choudhary2022recent}}

%\cite{ziletti2018insightful}\cite{modarres2017neural}\cite{yang2021deep}

% In ML for crystal studies, image representations of crystals often cannot precisely describe the entire crystal structure as accurately as geometric graphs and text. 

% Therefore, 



Crystal image representations are generated through methods such as diffraction imaging and scanning electron microscopy (SEM), etc~\cite{ziletti2018insightful,yang2021deep,choudhary2022recent}.
Diffraction images, obtained via experiments like X-ray diffraction (XRD), electron diffraction, or neutron diffraction, unveil the atomic arrangement and periodic structure within the crystal. Conversely, SEM images, captured using a scanning electron microscope, provide detailed insights into the surface morphology and structure of crystalline materials. These representations are instrumental in executing specific tasks such as defect detection and classification \cite{ziletti2018insightful, yang2021deep}.

%Often these tasks generalize across many different imaging modalities, spanning optical microscopy (OM), scanning electron microscopy (SEM) techniques, scanning probe microscopy (SPM, as in scanning tunneling microscopy (STM) or atomic force microscopy (AFM), and transmission electron microscopy (TEM) variants, including scanning transmission electron microscopy (STEM).
%The two-dimensional diffraction fingerprint
%STM-images Scanning tunneling microscopy images

\subsection{Spectra Representations}


% The collision of electromagnetic radiation with materials leads to an interaction that is quantified by the radiation's wavelength or frequency, ultimately yielding a spectroscopic signal. The spectra data are typically acquired via X-ray diffraction (XRD) and Raman spectroscopy~\cite{el2019raman,lee2020deep,choudhary2022recent}. XRD spectra, graphically depicted as plots of X-ray intensity versus the angle between the incident and diffracted beams, furnish quantitative information concerning crystal structure parameters, including peak positions and intensities, which correspond to interplanar spacings and crystallite sizes. On the other hand, Raman spectra, obtained by measuring the frequency shift of scattered light, provide characteristic information regarding molecular vibrations and crystal structure, thereby enabling the identification of chemical composition and crystal structure. By analyzing spectra data, researchers can gain an insightful understanding of the composition, structure, and dynamic properties of materials, thereby providing a nuanced comprehension of their intrinsic characteristics. 


The interaction between electromagnetic radiation and materials results in a quantifiable spectroscopic signal, dependent on the radiation's wavelength or frequency. Spectra data are commonly acquired through XRD and Raman spectroscopy~\cite{el2019raman, lee2020deep, choudhary2022recent}. XRD spectra, illustrated as plots of X-ray intensity against the angle between the incident and diffracted beams, offer quantitative information regarding crystal structure parameters, such as peak positions and intensities, which correspond to interplanar spacings and crystallite sizes. Conversely, Raman spectra, obtained by measuring the frequency shift of scattered light, provide characteristic information about molecular vibrations and crystal structures, thereby facilitating the identification of chemical composition and crystal structure. By analyzing spectra data, researchers can attain a comprehensive understanding of the composition, structure, and dynamic properties of materials, leading to an in-depth comprehension of their intrinsic characteristics.



\section{Fundamental Deep Learning Models}

% \zhong{Please reorganize the part as the following comments}


In this section, we will first briefly introduce some foundational knowledge commonly utilized in the study of crystalline materials. Following this, we will present basic machine learning models widely used in deep learning-driven material science, including convolutional neural networks, geometric GNNs, language models, and diffusion models.




\subsection{Geometric Graph Neural Networks}


Geometric graph neural networks (GGNNs) are specifically designed to handle the complex geometric and topological relationships within the graph-structured data. These networks are particularly suited for understanding and analyzing data that can be represented as graphs of 3D shapes, such as proteins, molecules, and crystalline materials. The key design principles of GGNNs are rooted in the principles of message-passing mechanism and aggregation. Through various message-passing mechanisms, GGNNs exchange and update information between neighboring nodes on the graph. Each node, utilizing its current embedding and the messages received from its nearest neighbors, computes an updated embedding that encapsulates the local information and structural context of the node. Aggregation performs local updates to node features by aggregating information from its immediate neighbors. Specifically, in GGNNs, message passing encodes not only node information but also edge and direction information. This is because crystalline materials exhibit symmetries of translations, rotations, and/or reflections, by incorporating the edge and direction information, the representation extracted by GGNNs can be equivariant or invariant to the group defined on the transformations, such as translations, rotations, and/or reflections. The concepts of group, equivariance, and invariance are provided in Box 1, and the design principles of message-passing mechanisms and aggregation are detailed in Box 2.

% This process allows the network to propagate and refine geometric information across the graph, capturing the spatial arrangement of nodes.


% graph convolution and message passing. Graph convolutional layers, inspired by CNNs, 




% By defining symmetry, we say that the model is invariant or equivariant to a set of transformations, such as translations, rotations, and/or reflections. 



\begin{tcolorbox} [breakable,boxrule=.2mm,arc = 0mm, outer arc = 0mm,left=0.2mm,right=0.2mm,top=0.3mm,bottom=0.3mm]
\noindent \textbf{Box 1 | Group, Equivariance and Invariance.}\tcblower\\
\textbf{Group~\cite{han2024survey}}\\ A group $G$ is a set of transformations with a binary operation “$\cdot$” that satisfies the following properties: (i) Closure: $\forall a,b\in G,a\cdot b\in G$; (ii) Associativity: $\forall a,b,c\in G,(a\cdot b)\cdot c=a\cdot(b\cdot c)$; (iii) Identity element: there exists an identity element $e\in G$ such that $\forall a\in G,a\cdot e=e\cdot a=a$; (iv) Inverses: there exists an identity element $e\in G$ such that $\begin{aligned}\forall a\in G,\exists b\in G,a\cdot b=b\cdot a=e\end{aligned}$, where the inverse $b$ is denoted as $a^{-1}$. Here are some groups commonly used in crystal research.
\begin{enumerate}
\item $E(d)$ is an Euclidean group comprising rotations, reflections, and translations, acting on $d$-dimension vectors.
\item $O(d)$ is an orthogonal group,  consisting of rotations and reflections, acting on d-dimension vectors.
\item $SE(d)$ is a special Euclidean group, which includes only rotations and translations.
\item $SO(d)$ is a special orthogonal group, consisting exclusively of rotations.
\item $S_N$ is a permutation group, whose elements are permutations of a given set consisting of N elements.
\end{enumerate}



\textbf{Equivariance}\\ Let $\mathcal{X}$ and $\mathcal{Y}$ be the input and output variables, respectively. The function $f:\mathcal{X}\to\mathcal{Y}$ is called equivariant with respect to a group $G$ if applying any transformation from $G$ to the input results in an identical transformation to the output. Formally, the function $f:\mathcal{X}\to\mathcal{Y}$ is $G$-equivariant if it commutes with any transformation in $G$, i.e., $\phi(g\cdot x)=g\cdot\phi(x),\forall g\in G$. By implementing the group operation $\cdot$ with group representation, can be rewritten as: $\phi(\rho_{\mathcal{X}}(g)x)=\rho_{\mathcal{Y}}(g)\phi(x),\forall g\in G$, where $\rho_{\mathcal{X}}(\cdot)$ and $\rho_{\mathcal{Y}}(\cdot)$ are the group representations in the input and
output spaces, respectively. 

\textbf{Unit Cell E(3) Equivariance}\\ In crystalline materials, we particularly consider the equivariance of unit cells. In the Cartesian coordinate system, for a function $f:(\mathbf{A},\mathbf{X},\mathbf{L})\to\mathcal{Y}\in \mathbb{R}^n$, if it is unit cell $SO(3)$ equivariant, then we have $\mathbf{Q}f(\mathbf{A},\mathbf{X},\mathbf{L}) = f(\mathbf{A},\mathbf{Q}\mathbf{X}+\boldsymbol{b},\mathbf{Q}\mathbf{L})$, where $\mathbf{Q}\in\mathbb{R}^{n \times n}$ is an arbitrary  rotation matrix and $\boldsymbol{b}\in\mathbb{R}^{n}$ is a translation vector.
%Intuitively, regardless of whether applying rotations and reflections to the position matrix $\mathbf{X}$ and lattice matrix $\mathbf{L}$ representing the 3D structure, or only applying translations to the spatial positions, the output of the function $f$ remains unchanged. In the context of crystal structure research, the function $f$ can be seen as the model under investigation. Since the same crystal at different positions in space does not result in a change in its properties, the E(3) invariance of $f$ significantly enhances the model's generalization ability.

% In addition, permutation equivariance w.r.t the atom order is also involved.

\textbf{Permutation Equivariance}\\ If function $f:(\mathbf{A},\mathbf{X},\mathbf{L})\to\mathcal{Y}\in \mathbb{R}^n$ is permutation equivariant, then we have $\mathbf{P}f(\mathbf{A},\mathbf{X},\mathbf{L}) = f(\mathbf{P}\mathbf{A},\mathbf{P}\mathbf{X},\mathbf{L})$, where $\mathbf{P}\in\{0,1\}^{n\times n}$ is a permutation matrix (represent the operation of adjusting the atom order). Naturally, when constructing crystal data $\mathbf{X}$, different node permutation orders will result in different representations of the crystal. However, in reality, these different representations correspond to the same crystal.

\textbf{Invariance}\\ Similar to Equivariance in Definition 2, the function $f:\mathcal{X}\to\mathcal{Y}$ is called invariant with respect to a group $G$. If any transformation is to the input, the output remains unchanged. In form, the function $f:\mathcal{X}\to\mathcal{Y}$ is $G$-invariant if it commutes with any transformation in $G$, $\phi(g\cdot x)=\phi(x),\forall g\in G$.
By implementing the group operation $\cdot$ with group representation, this can be rewritten as: $\phi(\rho_{\mathcal{X}}(g)x)=\phi(x),\forall g\in G$, where $\rho_{\mathcal{X}}(\cdot)$ and $\rho_{\mathcal{Y}}(\cdot)$ are the group representations in the input and output space, respectively. Next, we give a concrete example of Invariance in crystal research.

% Similarly, we consider the invariance of unit cells.


\textbf{Unit Cell E(3) Invariance}\\ We particularly consider the invariance of unit cells. For a function $f:(\mathbf{A},\mathbf{X},\mathbf{L})\to\mathcal{Y}$, if it is invariant under the $E(3)$ group, then we have $f(\mathbf{A},\mathbf{X},\mathbf{L}) = f(\mathbf{A},\mathbf{Q}\mathbf{X}+\boldsymbol{b},\mathbf{Q}\mathbf{L})$, where $\mathbf{Q}\in\mathbb{R}^{3 \times 3}$ is a rotation and reflection matrix and $\boldsymbol{b}\in\mathbb{R}^{3}$ is a translation vector.
%Intuitively, regardless of whether applying rotations and reflections to the position matrix $\mathbf{X}$ and lattice matrix $\mathbf{L}$ representing the 3D structure, or only applying translations to the spatial positions, the output of the function $f$ remains unchanged. In the context of crystal structure research, the function $f$ can be seen as the model under investigation. Since the same crystal at different positions in space does not result in a change in its properties, the E(3) invariance of $f$ significantly enhances the model's generalization ability.

% In addition, periodic invariance w.r.t the lattice parameters is involved.


\textbf{Periodic Invariance}\\ For a crystal, maintaining the shape of the unit cell while scaling the unit cell's size or shifting the unit cell to move the periodic boundary will result in a transformation of the atomic coordinates within the unit cell. Therefore, this periodicity leads to different crystal data representations for the same crystal. Consequently, models applied to crystal data also need to be periodic invariant. If a function $f:(\mathbf{A},\mathbf{X},\mathbf{L})\to\mathcal{X}$ exhibits periodic invariance,  $f(\mathbf{A},\mathbf{X},\mathbf{L})=f(\Phi(\hat{\mathbf{A}},\hat{\mathbf{X}},\boldsymbol{\alpha}\mathbf{L},\mathrm{p}),\boldsymbol{\alpha}\mathbf{L})$, where $\Phi:(\hat{\mathbf{A}},\hat{\mathbf{X}},\mathbf{L},\mathrm{p})\to(\mathbf{A},\mathbf{X})$ represents the abstract generating function of the unit cell and $\mathrm{p}$ is a corner point. $\alpha\in\mathbb{N}_{+}^{3}$ is a scalar that pertains to the scaling of unit cell size.

\begin{comment}
\begin{figure}[ht] 
  \centering   
  \includegraphics[width=4.3in]{fig/Periodic.pdf}
  \caption{\textbf{Illustration of periodic invariance.} Purple lines are the edges between nodes inside a unit cell. Red points are the corner points of the unit cells. For example, $p_1$ and $p_2$ are for unit cells in \textbf{a} and \textbf{b}, respectively, but $p_1$ (or $p_2$) has different coordinates in \textbf{a} and \textbf{b}. (figure obtained from REF.\cite{yan2022periodic}).}
  \label{fig:Periodic}
\end{figure} 
\end{comment}
% In certain diffusion-based crystal generation methods \cite{jiao2023crystaliclr}, to ensure the E(3) invariance of the model, the denoising network in the diffusion reverse process is required to be E(3) equivariant (or O(3) equivariant, as translational operations can be avoided through a zero-center-of-mass system). That is, $\mathbf{Q}f(\mathbf{A},\mathbf{C},\mathbf{L}) = f(\mathbf{A},\mathbf{Q}\mathbf{C}+\boldsymbol{b},\mathbf{Q}\mathbf{L})$.

% 

\textbf{Permutation Invariance}\\ Similarly, we consider the permutation invariance w.r.t the atom order. 
%a permutation matrix $\mathbf{P}\in\{0,1\}^{N\times N}$ 
If function $f:(\mathbf{A},\mathbf{X},\mathbf{L})\to\mathcal{X}$ is permutation invariant, then we have $f(\mathbf{A},\mathbf{X},\mathbf{L}) = f(\mathbf{P}\mathbf{A},\mathbf{P}\mathbf{X},\mathbf{L})$, where $\mathbf{P}$ is a permutation matrix. 
\end{tcolorbox}


\begin{tcolorbox} [breakable,boxrule=.2mm,arc = 0mm, outer arc = 0mm,left=0.2mm,right=0.2mm,top=0.3mm,bottom=0.3mm]
\noindent \textbf{Box 2 | Principles of Message Passing Mechanism.}\tcblower
The message passing mechanism processes graph-structured data by exchanging each node's information with its neighboring nodes through edges; specifically, each node aggregates the representation information from its neighboring nodes using an aggregation function. The aggregated information is then treated as the message of the node. The node feature update function combines the message with the node's own representation to generate a new representation for the node. By iteratively applying the message-passing through multiple network layers, the node representations can incorporate more comprehensive graph structure information. Formally, the message-passing mechanism can be expressed as follows \cite{gilmer2017neural}:
\begin{equation}
m_{ij}=\phi_{\mathrm{msg}}\left(h_{i}^{(l-1)},h_{j}^{(l-1)},e_{ij}\right),\quad
h_{i}^{(l)}=\phi_{\mathrm{upd}}\left(h_{i}^{(l-1)},\{m_{ij}\}_{j\in\mathcal{N}_{i}}\right),
\end{equation}
where $\phi_{\mathrm{msg}}(\cdot)$ and $\phi_{\mathrm{upd}}(\cdot)$ represent the message calculation and feature update functions, respectively. $h_{i}^{(l-1)}$ and $h_{j}^{(l-1)}$ are the node features of the $i$-th and $j$-th nodes, respectively, in the $(l-1)$-th layer. $h_{i}^{(l)}$ represents the node feature of the $i$-th node in the $l$-th layer. $e_{ij}$ denotes the edge features between the two nodes, and $m_{ij}$ represents the computed message.
\end{tcolorbox}



% \vspace{0.5cm}
% \textbf{Invariance and Equivariance}

% Unlike molecular, crystal are composed of repeating unit cells on a regular lattice in 3D space. Therefore, crystals exhibit different structural distribution symmetries in 3D space.
%, such as permutation invariance, unit cell E(3) invariance, and periodic invariance. 
%Next, we will introduce these properties in the Cartesian coordinate system.

%If the function $f$ is the proposed or studied model, the permutation invariance of $f$ can enhance the model's generalization ability.

%If function $f:(\mathbf{A},\mathbf{C},\mathbf{L})\to\mathcal{X}$ is permutation invariant, then we have $f(\mathbf{A},\mathbf{C},\mathbf{L}) = f(per(\mathbf{A}),per(\mathbf{C}),\mathbf{L})$, where $per(\cdot)$ represents the operation of adjusting the atom order. Accordingly, if function $f$ is permutation equivariant, then we have $per(f(\mathbf{A},\mathbf{C},\mathbf{L})) = f(per(\mathbf{A}),per(\mathbf{C}),\mathbf{L})$. Naturally, when constructing crystal data $\mathbf{C}$, different node permutation orders will result in different representations of the crystal. However, in reality, these different representations correspond to the same crystal. 
%If the function $f$ is the proposed or studied model, the permutation invariance of $f$ can enhance the model's generalization ability.


% \subsection{Geometric GNNs}


% \textcolor{cyan}{A crystal structure is a periodic, infinite arrangement of unit cells composed of atoms in 3D Euclidean space. 
% To enable GNNs to handle such infinite structures, it is typically necessary to employ graph construction methods that represent the interactions between infinite crystal structures and atoms using finite graph data. Subsequently, GNNs can utilize the graph data to analyze the crystal structures.}

% \vspace{0.5cm}
% \textcolor{cyan}{\textbf{Crystal Graph Construction}}

% A multi-edge graph is a common method used to describe the structure and relationships within crystals \cite{xie2018crystal}.
% In a multi-edge graph, nodes represent atoms and all their copies within the infinite 3D space of the crystal, while edges represent the connections between atoms in the crystal. The multi-edge connections between nodes reflect the periodicity of the crystal, connecting atoms from different unit cells. Specifically, assuming that a crystal $\mathbf{M}$ can be transformed into a crystal graph $\mathbf{G}(\mathbf{V},\mathbf{E})$. $\mathbf{V}$ denotes the set of nodes $v_i$ in the crystal graph, where $v_i$ contains atomic features, i.e. $v_i=(\boldsymbol{a}_{i},\hat{\boldsymbol{p}}_i)$.
% $\mathbf{E}$ represents the set of edges $e_{ij}$ representing spatial connections between atoms. In the multi-edge Graph, edges $e_{ij}$ are typically constructed based on the Euclidean distance $d_{ij}$ between atoms $v_i$ and $v_j$. For
% $d_{ij}=||\boldsymbol{p}_{j}+k_{1}\boldsymbol{l}_{1}+k_{2}\boldsymbol{l}_{2}+k_{3}\boldsymbol{l}_{3}-\boldsymbol{p}_{i}||_{2}\leq R$,
% when the Euclidean distance $d_{ij}$ between atoms $v_i$ and $v_j$ is less than a given radius $R$, an edge $e_{ij}$ with the initial edge feature $d_{ij}$ is created between $v_i$ and $v_j$. 
% Different values of $\boldsymbol{k}=[k_{1},k_{2},k_{3}]\in\mathbb{R}^{3}$ represent different edges between nodes $v_i$ and $v_j$.
% A simple demonstration of transforming a two-dimensional crystal structure diagram into a multi-edge graph is shown in Fig. \ref{fig:multi-edge-graph}.

% \begin{figure}[h] 
%   \centering   
%   \includegraphics[width=3.3in]{fig/multi-edge-graph.pdf}
%   \caption{Illustration of the multi-edge graph construction. (figure obtained from \cite{yan2024complete}).}
%   \label{fig:multi-edge-graph}
% \end{figure} 


% In some AI for Crystal research \cite{wang2024conformal,yan2024complete}, the k-connected graph is also used to describe crystal structures. In the k-connected graph, the construction of nodes is the same as in the multi-edge graph, while the construction of edges is achieved by connecting an atom to its k nearest neighboring atoms.


% \vspace{0.5cm}

% \textbf{Geometric GNNs}. After introducing the basic concept, we give the general form of Geometric GNNs. 



% Typically, geometric GNNs can be classified into two classes: invariant and equivariant GNNs.
% % In the field of crystal research, various tasks, such as predicting crystal properties, require models that exhibit invariance properties in order to enhance their generalization to crystal structures. Therefore, invariant GNNs have found extensive applications in such tasks. 
% The current mainstream invariant GNNs typically focus on E(3) invariance, often employing various invariant scalars in their message-passing mechanisms, such as relative distances and angles between edges. This approach aims to mitigate the effects of E(3) group transformations on spatial coordinates.
% Different from invariant GNNs that only update invariant features, equivariant GNNs simultaneously update invariant and equivariant features (like the coordinate), generating equivariant outputs while the input changes. Current mainstream equivariant GNN design approaches can be categorized into two types: scalarization-based and high degree steerable \cite{han2024survey}.
% Scalarization-based approaches translate 3D coordinates into invariant scalars, which is similar to the design of invariant GNNs, but it refines beyond invariant GNNs by further recovering the direction of the processed scalars for the update of equivariant features. The core idea of high degree steerable approaches is to utilize higher-order tensors to represent the features of nodes and edges in a graph. By applying steerable operations, such as rotations and reflections, these features are processed to ensure that the network remains equivariant to such transformations.%Specifically, high-degree steerable GNNs design appropriate convolutional kernels and feature transformations to ensure that the network's output remains stable under certain symmetry operations.

\subsection{Convolutional Neural Networks}

%Convolutional Neural Networks (CNNs) are a type of deep learning architecture that revolutionized image processing and computer vision tasks. CNNs can be applied to analyze crystalline materials in several ways, especially in aiding characterization, such as structure recognition, defect detection, and microstructure analysis. CNNs utilize convolutional layers to automatically detect spatial hierarchies in data. Convolutional operations involve sliding a convolutional kernel over the input data to compute local patterns. The convolution process allows the network to learn features from small local regions and gradually capture more complex patterns as the network deepens. After convolutional layers, pooling layers downsample the feature maps, retaining the most important information while reducing dimensionality. Common pooling methods include max pooling and average pooling. Pooling helps combat overfitting and reduces computational load. CNNs use activation functions like ReLU to introduce non-linearity into the model. In typical CNN architectures, the final layers are fully connected layers, which take the high-level features learned by the convolutional and pooling layers to make final predictions. The principles of each design in CNNs, including convolution, pooling, etc., are detailed in Box 2.
Convolutional Neural Networks (CNNs) represent a pivotal deep learning architecture that has revolutionized image processing and computer vision tasks. These networks can be effectively applied to the analysis of crystalline materials, particularly in facilitating characterization tasks such as structure recognition, defect detection, and microstructure analysis. CNNs employ convolutional layers to autonomously detect spatial hierarchies within data. Convolutional operations involve sliding a convolutional kernel over the input data to compute local patterns. This process enables the network to learn features from small local regions and progressively capture more complex patterns as the network deepens. Following the convolutional layers, pooling layers are used to downsample the feature maps, retaining the most critical information while reducing dimensionality. Common pooling methods include max pooling and average pooling, both of which help mitigate overfitting and decrease computational load. CNNs incorporate activation functions like ReLU to introduce non-linearity into the model. In standard CNN architectures, the final layers are fully connected layers, which utilize the high-level features learned by the convolutional and pooling layers to make final predictions. The principles of each design component in CNNs, including convolution, pooling, and activation functions, are elaborated in Box 3.

\begin{tcolorbox} [breakable,boxrule=.2mm,arc = 0mm, outer arc = 0mm,left=0.2mm,right=0.2mm,top=0.3mm,bottom=0.3mm]
\noindent \textbf{Box 3 | Principles of CNNs.}\tcblower
The core of CNNs is the combination of convolutional layers and pooling layers. The convolutional layer uses multiple convolutional kernels to compute different feature maps, thereby learning the feature representation of the input. Specifically, each neuron in a feature map has a receptive field, which is connected to the neighborhood of neurons in the previous layer \cite{rawat2017deep}. New feature maps can be obtained by convolving the input with the learned kernels and then applying an element-wise nonlinear activation function to the convolution result. This process is mathematically represented as follows
\begin{equation}
\mathbf{Y}_k=\sigma(\mathcal{W}_k*\mathbf{X}+b_k)
\end{equation}
where $\mathbf{Y}_k$ is the $k-$th output feature map; the input is denoted by $\mathbf{X}$; the convolutional filter related to the $k-$th feature map is denoted by $\mathcal{W}_k$; $b_k$ is the bias term of the $k-$th filter; $*$ is used for the convolution operation; and
$\sigma(\cdot)$ represents the nonlinear activation function.
Correspondingly, Pooling layers are placed between two convolutional layers and achieve translation invariance by reducing the resolution of feature maps. Formally, the max pooling layer selects the largest element within each receptive field such that $y_{k}^{i,j}=\max x_{k}^{m,n}, (m,n)\in\mathcal{R}_{ij}$, 
where $\mathcal{R}_{ij}$ is a local neighbourhood around location $(i,j)$ and $x_{k}^{m,n}$ denotes the element at location $(m,n)$. 
\end{tcolorbox}


\subsection{Language Models}

The evolution of language models within the domain of deep learning has witnessed remarkable progress over the past decade, particularly in the field of natural language processing~\cite{han2022survey,xiao2023transformers,zhang2023applications}.
%With the emergence of chemical languages, e.g., simplified molecular input line entry systems (SMILES~\cite{weininger1988smiles}), language models have also demonstrated tremendous potential in the field of science. 
Historically, recurrent neural networks (RNNs) and long short-term memory (LSTM) networks were the most common approaches for language modeling. 
These architectures processed text sequences sequentially, adeptly capturing temporal dependencies but often encountering difficulties with long-range context retention. The advent of transformer models marked a pivotal shift by employing self-attention mechanisms~\cite{vaswani2017attention}, which enabled parallel processing of entire input sequences and thus improved the modeling of long-range dependencies.
The transformer architecture consists of an encoder and a decoder, both composed of multiple layers. 
The encoder transforms an input sequence into a fixed-length vector, or embedding, which encapsulates the contextual and semantic information of the input. This embedding is then utilized by the decoder to generate the output sequence incrementally, with each step informed by attention to various segments of the input
One of the key innovations in transformer models is the multi-head self-attention mechanism, which allows the model to attend to different parts of the input with different "heads", each focusing on a different aspect of the information to understand the relationships between words and their context. The design principles of the transformer are detailed in Box 4.


% The Transformer  is a deep learning model that can achieve state-of-the-art performance in various tasks \cite{han2022survey,xiao2023transformers,zhang2023applications}. Given that the Transformer is a sequence-to-sequence model, by serializing crystal material data, it can naturally be applied to the field of crystal material research. 

%Researchers often use networks based on the Transformer architecture to predict the properties of crystal materials.
% When specifically applying the Transformer network structure, it is common to first perform embedding encoding on the node and edge features of the crystal graph. 
% For node features, GNNs are used for embedding encoding, such as using CGCNN~\cite{xie2018crystal} for node feature encoding in \cite{yan2024complete, yan2022periodic}. For edge features, radial basis function (RBF)~\cite{choudhary2021atomistic} is typically employed.


% Then, self-attention layers are applied to these embeddings to compute the query, key, and value \cite{vaswani2017attention}.



% The large language model (LLM) is a large-scale neural network model, typically based on the Transformer architecture, containing billions to trillions of parameters. 
In recent years, the development of large language models (LLMs) based on the transformer has been driven by the availability of massive amounts of data and the increasing computational power. Based on the transformer architecture, LLMs, often with hundreds or even trillions of parameters, have achieved remarkable performance on a wide range of language processing tasks \cite{zhao2023survey,deletang2023language}.
Typically, LLMs undergo a pre-training phase on vast corpora of text data, which enables them to discern and assimilate prevalent linguistic patterns. Subsequent fine-tuning on task-specific datasets further refines their performance and adaptability. Some notable examples of large language models include BERT~\cite{kenton2019bert}, OPT~\cite{zhang2022opt}, GPT~\cite{brown2020language}, Llama\cite{touvron2023llama}, etc. Recently, the surge in multimodal data generation within scientific domains, such as molecular structures, proteins, and genomes, has catalyzed the development of scientific LLMs designed to comprehend, interpret, and generate specialized scientific languages~\cite{zhang2024scientific}. These scientific LLMs include medical LLMs~\cite{chen2023meditron,peng2023study}, biological LLMs~\cite{madani2020progen,mansoor2021toward,hwang2024genomic}, chemical LLMs~\cite{zhou2023uni,chang2024bidirectional,wang2024explainable}, and comprehensive LLMs~\cite{beltagy2019scibert,hong2023diminishing,xie2023darwin}.

%even promoting self-driving laboratories~\cite{m2024augmenting,boiko2023autonomous}.




\begin{tcolorbox} [breakable,boxrule=.2mm,arc = 0mm, outer arc = 0mm,left=0.2mm,right=0.2mm,top=0.3mm,bottom=0.3mm]
\noindent \textbf{Box 4 | Principles of Transformers.}\tcblower
The core innovation of the Transformer is the self-attention mechanism. This allows the model to weigh the significance of different words in a sequence relative to one another. By calculating attention scores, the model can focus on particular parts of the input, enabling it to capture contextual relationships without relying on sequential processing. Specifically, through defining three learnable weight matrices $\mathbf{W}^{\mathbf{Q}}\in\mathbb{R}^{d\times d_q}$, $\mathbf{W}^{\mathbf{K}}\in\mathbb{R}^{d\times d_k}$, and $\mathbf{W}^{\mathbf{V}}\in\mathbb{R}^{d\times d_v}$,the input embeddings $\mathbf{X}\in\mathbb{R}^{n\times d}$ are linearly transformed to three parts, i.e., queries $\mathbf{Q}\in\mathbb{R}^{n\times d_q}$, keys $\mathbf{K}\in\mathbb{R}^{n\times d_k}$, values $\mathbf{V}\in\mathbb{R}^{n\times d_v}$, where $\mathbf{Q}=\mathbf{X}\mathbf{W}^{\mathbf{Q}}$, $\mathbf{K}=\mathbf{X}\mathbf{W}^{\mathbf{K}}$, $\mathbf{V}=\mathbf{X}\mathbf{W}^{\mathbf{V}}$, and $d$, $d_q$, $d_k$, $d_v$ are the dimensions of inputs, queries, keys and values ($d_k=d_q$), respectively. The output of the self-attention layers is,
\begin{equation}
    \mathrm{attention}(\mathbf{Q},\mathbf{K},\mathbf{V})=\mathrm{softmax}\left(\frac{\mathbf{Q}\mathbf{K}^T}{\sqrt{d_q}}\right)\mathbf{V}.
    \end{equation}
Afterward, the output of the $H$ different self-attention layers is then concatenated and are linearly transformed to multi-head attention output, $
\mathrm{MultiHeadAttnoutput}=\mathrm{Concat} (head_1,\cdots,head_H)\mathbf{W}^{\mathbf{Z}}$,
where $head_i=\mathrm{attention}(\mathbf{Q_i},\mathbf{K_i},\mathbf{V_i})$, $\mathbf{W}^{\mathbf{Z}}\in\mathbb{R}^{H\cdot d_v\times d}$.
Besides, a residual connection module followed by a layer normalization module is inserted around each module. That is, $\mathbf{H}^{\prime} = \mathrm{LayerNorm}(\mathrm{Attn}(\mathbf{X}) + \mathbf{X}), \quad
\mathbf{H} = \mathrm{LayerNorm}(\mathrm{FFN}(\mathbf{H}') + \mathbf{H}')$, where $\mathrm{Attn(\cdot)}$ denotes multi-head attention module,
$\mathrm{LayerNorm(\cdot)}$ denotes the layer normalization operation, and
$\mathrm{FFN(\cdot)}$ denotes the feed-forward network as
$\mathrm{FFN}(\mathbf{H}')=\mathrm{ReLU}(\mathbf{H}'\mathbf{W}_1+\mathbf{b}_1)\mathbf{W}_2+\mathbf{b}_2$, where $\mathbf{W}_1$, $\mathbf{W}_2$, $\mathbf{b}_1$, $\mathbf{b}_2$ are trainable parameters.
\end{tcolorbox}



% Due to their powerful representation capabilities, LLMs possess strong transfer learning abilities and can extrapolate various types of data \cite{deletang2023language}.





% In the research of crystalline materials, by encoding crystal structure information as text or other sequence representations, 
%LLMs can learn to predict the physical and chemical properties of materials \cite{}. 


% LLMs can also generate new crystal structures by learning patterns from existing crystal structures \cite{gruver2024finetuned}. 
% In practical applications, researchers typically use parameter efficient fine tuning (PEFT) \cite{ding2023parameter} on pre-trained models because it requires fewer training samples and training parameters, significantly reducing computational costs. Common pre-trained models include
% % GPT \cite{brown2020language}, 
% Galactica \cite{taylor2022galactica}, OPT \cite{zhang2022opt}, and LLaMA \cite{touvron2023llama}.

\subsection{Diffusion Models}


%Deep generative models are neural networks trained to approximate complicated, high-dimensional probability distributions using a large number of samples. These models are widely used in generating realistic data such as images, audio, and scientific data. Traditional deep generative models like Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs) learn a mapping from a low-dimensional latent space to the data distribution and generate new data instances by sampling latent variables from the latent space. However, they are prone to falling into mode collapse or unstable training issues. Recently, diffusion models offered advantages over traditional deep generative models by providing high-fidelity samples, training stability, and adaptability to data complexity. 

Deep generative models are advanced neural networks designed to approximate intricate, high-dimensional probability distributions, using extensive sample datasets. These models have found broad applications in generating realistic data across various domains, including images, audio, and scientific data. Traditional deep generative frameworks, such as Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs), operate by learning a mapping from a low-dimensional latent space to the data distribution, and generate new data instances by sampling from this latent space. However, these models often encounter challenges such as mode collapse and training instability. 

Recently, diffusion models offered advantages over traditional deep generative models by providing high-fidelity samples, training stability, and adaptability to data complexity. 
Diffusion models, inspired by the principles of particle spread in physics, are probabilistic generative models that generate data by gradually adding noise and reconstructing data by progressively removing the noise through a reverse process~\cite{yang2023diffusion}. 
The functioning of diffusion models involves a two-phase process: the forward diffusion process and the reverse diffusion process. 
In the forward diffusion phase, noise is incrementally added to the data, systematically transforming it into a simpler distribution. This phase is mathematically represented as a sequence of states, each representing a progressively noisier version of the preceding state. Conversely, the reverse diffusion process learns to reconstruct the original data by progressively removing the noise. This reconstruction is facilitated by a neural network that estimates the denoised state from the noisy input. The detailed working principle can be found in Box 5.



\begin{tcolorbox} [breakable,boxrule=.2mm,arc = 0mm, outer arc = 0mm,left=0.2mm,right=0.2mm,top=0.3mm,bottom=0.3mm]
\noindent \textbf{Box 5 | Principles of Diffusion Models.}\tcblower
A diffusion model is defined by a forward process that gradually destroys data $\mathbf{x}_0 \sim q(\mathbf{x}_0)$ over $T$ timesteps.
\begin{equation}
   q(\mathbf{x}_{1:T}|\mathbf{x}_0)=\prod_{t=1}^{T} q(\mathbf{x}_{t}|\mathbf{x}_{t-1}), \quad
  q(\mathbf{x}_{t}|\mathbf{x}_{t-1})=\mathcal{N}(\mathbf{x}_{t};\sqrt{1-\beta_t}\mathbf{x}_{t-1},\beta_t\mathbf{I}),
\end{equation}
and a parameterized reverse process $p_{\theta}(\mathbf{x}_0)=\int p_{\theta}(\mathbf{x}_{0:T})d \mathbf{x}_{1:T}$, where
\begin{equation}
   p_{\theta}(\mathbf{x}_{0:T})=p(\mathbf{x}_{T}) \prod_{t=1}^{T} p_{\theta}(\mathbf{x}_{t-1}|\mathbf{x}_{t}), \quad
   p_{\theta}(\mathbf{x}_{t-1}|\mathbf{x}_{t})=\mathcal{N}(\mathbf{x}_{t-1};\mu_{\theta}(\mathbf{x}_{t},t),\Sigma_{\theta}(\mathbf{x}_t,t)).
\end{equation}
The forward process hyperparameters $\beta_t$ are set so that $\mathbf{x}_{T}$ is approximately distributed according to a standard normal distribution, so $p(\mathbf{x}_{T})$ is set to a standard normal prior as well. The reverse process is trained to match the joint distribution of the forward process by optimizing the evidence lower bound (ELBO) $-L_{\theta}(\mathbf{x}_{0})\leq \log p_{\theta} (\mathbf{x}_{0})$,
\begin{equation}
L_{\theta}(\mathbf{x}_{0})=\mathbb{E}\left[\log \frac{q(\mathbf{x}_{T}|\mathbf{x}_{0})}{p_{\theta} (\mathbf{x}_{T})}+\sum_{t>1} \log \frac{q(\mathbf{x}_{t-1}|\mathbf{x}_{0},\mathbf{x}_{1})}{p_{\theta} (\mathbf{x}_{t-1}|\mathbf{x}_{t})}
-\log p_{\theta}(\mathbf{x}_{0}|\mathbf{x}_{1}) \right].
\end{equation}
However, directly optimizing this objective is known to suffer serious training instability, a modified loss instead of the ELBO can be optimized,
\begin{equation}
L_{DM}(\theta)=\mathbb{E}_{\mathbf{x}_0,\epsilon\sim\mathcal{N}(0,\mathbf{I}),t}\left[ ||\epsilon-\epsilon_{\theta}(\sqrt{\Tilde{\alpha}_t}\mathbf{x}_0+\sqrt{1-\Tilde{\alpha}_t}\epsilon,t)||^2\right].
\end{equation}
\end{tcolorbox}

% To ensure the reverse denoising process accurately reconstructs the original data, Diffusion Models utilize variational inference to optimize model parameters. By maximizing the ELBO, the model can learn to generate realistic samples from noise.
% When specifically applied to crystal generation, diffusion models often generate the geometric graph representation of the crystal \cite{jiao2023crystaliclr,jiao2024space}.



\begin{table*}[htbp]
  \centering
  \caption{Summary of Models for Material Property Prediction}
      \rowcolors{2}{gray!25}{white}
\renewcommand\arraystretch{1.35}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllll}
    \toprule
    Methods & Data Representation & Base Models & Physical Knowledge & The Predicted Properties\\
    \midrule

    SchNet~\cite{schutt2018schnet,schutt2017schnet} &  Geometric Graph  &Geometric GNN  &  -   &Formation Energy, Band gap, etc\\  
    
    CGCNN~\cite{xie2018crystal} &Geometric Graph &Geometric GNN & - & Total Energy, Band gap, etc\\


    
    MEGNET~\cite{chen2019graph} & Geometric Graph  & Geometric GNN &  Global state, e.g. temperature  &Formation Energy, Band gap, etc\\ 
        
    GATGNN~\cite{louis2020graph} & Geometric Graph  &Geometric GNN &   -  &Formation Energy, Band gap, etc \\ 
        
    ALIGNN~\cite{choudhary2021atomistic,kaundinya2022prediction} & Geometric Graph  & Atomistic Line GNN &  -   &Electron DOS, Band gap, etc\\ 
    

    ECN~\cite{kaba2022equivariant} & Geometric Graph &Geometric GNN & Space group  &Formation Energy, Band gap, etc\\
    PotNet~\cite{lin2023efficient} & Geometric Graph &Geometric GNN &  Interatomic potentials &Total Energy, Band gap, etc\\
    CrysGNN~\cite{das2023crysgnn} & Geometric Graph &Geometric GNN &  - &Total Energy, Band gap, etc\\


    ETGNN~\cite{zhong2023general} & Geometric Graph & Geometric GNN &   -  &Dielectric, Piezoelectric, and Elastic tensors\\   
    

    GMTNet~\cite{taniai2024crystalformer} &  Geometric Graph & Geometric GNN &   Space group  &Dielectric, Piezoelectric, and Elastic tensors\\   
    
    ComFormer~\cite{yan2024complete} &   Geometric Graph & Transformer &  -& Total Energy, Band gap, etc\\        
    Crystalformer (ICLR)~\cite{taniai2024crystalformer} &  Geometric Graph & Transformer &   Neural potential summation &Total Energy, Band gap, etc\\        
    Crystalformer (AAAI)~\cite{wang2024conformal} &  Geometric Graph & Transformer  &   - &Total Energy, Band gap, etc\\ 
    %Harmonic mapping with minimized Dirichlet energy
    E(3)NN~\cite{chen2021direct} &  Geometric Graph&Geometric GNN  &   - & Phonon DOS, Electron DOS, etc\\ 
    DOSTransformer~\cite{lee2024density} & Geometric Graph & Transformer  &   Energy
    level of material & Phonon DOS, Electron DOS, etc\\ 


    
    Matformer~\cite{yan2022periodic} &  Geometric Graph & Transformer  &  -& Total Energy, Band gap, etc\\ 
    CrysDiff~\cite{song2024diffusion} &  Fractional coordinate & Diffusion &  Space group  & Total Energy, Band gap, etc\\
    Uni-MOF~\cite{wang2024comprehensive} &  Text-CIFs & Transformer &  - & Adsorption properties\\

    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table*}%



% The forward process posteriors $q(\mathbf{x}_{t-1}|\mathbf{x}_{0},\mathbf{x}_{1})$ and marginals $q(\mathbf{x}_{t}|\mathbf{x}_{0})$ are Gaussian, and the KL divergences in the ELBO can be calculated in closed form. Thus it is possible to train the diffusion model by taking stochastic gradient steps on random terms.

% As suggested, we use the reverse process parameterizations
% \begin{equation}
% \begin{split}
% & \mu_{\theta}(\mathbf{x}_{t},t)=\frac{1}{\sqrt{\alpha_t}}(\mathbf{x}_{t}-\frac{\beta_t}{\sqrt{1-\Tilde{\alpha}_t}}\epsilon(\mathbf{x}_{t},t))\\
% & \Sigma_{\theta}^{ii}(\mathbf{x}_t,t)=\exp({\log \Tilde{\beta}_t+(\log \beta_t-log \Tilde{\beta}_t)v_{\theta}^{i}(\mathbf{x}_t,t)})
% \end{split}
% \end{equation}
% where $\alpha_t=1-\beta_t$, $\Tilde{\alpha}_t=\prod_{s=1}^{t}\alpha_s$, and $\Tilde{\beta}_t=\frac{1-\Tilde{\alpha}_{t-1}}{1-\Tilde{\alpha}_t}\beta_t$. 



\section{Material Discovery Tasks}

\subsection{Physicochemical Property Prediction}
%Predicting the properties of crystalline materials is a complex and extensive field that involves various theories and experimental methods. It remains a challenging task due to the numerous factors involved. Recently, deep learning methods have made a significant impact on the study of crystalline materials, and an increasing number of researchers have developed deep learning models for predicting the properties of these materials \cite{yan2024complete,taniai2024crystalformer,song2024diffusion,lee2024density,yan2022periodic,lin2023efficient}. These methods leverage artificial neural networks to capture the mapping relationship between crystal representation data and property information from large datasets, enabling them to make predictions for a wide range of material properties. Currently, popular methods in this field can be categorized based on neural network types, including GNN-based methods, transformer-based methods, and diffusion-based methods.

Predicting the properties of crystalline materials is a multifaceted and intricate field that encompasses a broad array of theoretical frameworks and experimental methodologies. The complexity of this task is attributed to the numerous variables and interactions involved. Recently, deep learning techniques have significantly advanced the study of crystalline materials, with an increasing number of researchers developing sophisticated models to forecast material properties \cite{yan2024complete,taniai2024crystalformer,song2024diffusion,lee2024density,yan2022periodic,lin2023efficient}. These methods utilize artificial neural networks to discern the mapping between crystal representation data and property information derived from extensive datasets, thus facilitating predictions across a diverse spectrum of material properties. Presently, prominent approaches in this area are categorized into neural network types, including GNN-based methods, transformer-based methods, and diffusion-based methods.

\subsubsection{Geometric Graph-Based Prediction}
%Due to the periodic and infinite arrangement of atoms in a crystal structure within 3D Euclidean space, GNN-based property prediction methods require the use of graph construction methods to represent the infinite crystal structure and the interactions between atoms with finite graph data. Specifically, nodes in the graph represent atoms and all their copies within the infinite 3D space of the crystal, while edges represent the connections between atoms in the crystal. The multi-edge connections between nodes reflect the periodicity of the crystal, connecting atoms from different unit cells. After constructing the graph, GNN-based methods perform supervised learning with the GNN and the associated property dataset. The trained GNN is then used for property prediction.
Due to the inherently periodic and infinite arrangement of atoms in a crystal structure within 3D Euclidean space, GNN-based property prediction methods necessitate sophisticated graph construction techniques to effectively represent the infinite lattice and its atomic interactions using finite graph data. In this framework, nodes in the graph correspond to atoms and their periodic replicas across the crystal's 3D expanse, while edges delineate the interactions between these atomic entities. The multiple edge connections between nodes capture the crystal's periodicity by linking atoms across distinct unit cells. Following the graph construction, GNN-based methods employ supervised learning to train the network on a dataset of crystal properties. Once trained, the GNN is leveraged to predict properties of crystalline materials based on the learned representations and interactions encoded in the graph.

An exemplary application of GNNs in this context is SchNet, initially designed for simulating quantum interactions in molecules using continuous-filter convolutional layers~\cite{schutt2017schnet}. This method directly models interactions between atoms utilizing distance information, thereby providing rotationally invariant energy predictions. For crystalline materials, which are atomistic systems characterized by periodic boundary conditions (PBCs), SchNet can directly apply the PBCs to the filter-generating network by summing over all periodic images within the given cutoff~\cite{schutt2018schnet}. Since the periodic filter is rotationally equivariant, this adaptation preserves the rotational invariance of the final property predictions.


CGCNN also is a pioneering GNN framework specifically designed for handling crystal structures~\cite{xie2018crystal}. This model was the first to represent crystal structures as multi-edge graphs where nodes represent atoms and edges represent interactions between atoms. In the multi-edge graph proposed by CGCNN, nodes represent atoms and all their copies within the infinite 3D space of the crystal, while edges represent the connections between these atoms. The multi-edge connections between nodes reflect the periodicity of the crystal, connecting atoms from different unit cells.

Specifically, assuming that a crystal $\mathbf{M}$ can be transformed into a crystal graph $\mathbf{G}(\mathbf{V},\mathbf{E})$. $\mathbf{V}$ denotes the set of nodes $v_i$ in the crystal graph, where $v_i$ contains atomic features, i.e. $v_i=(\boldsymbol{a}_{i},\hat{\boldsymbol{p}}_i)$.
$\mathbf{E}$ represents the set of edges $e_{ij}$ representing spatial connections between atoms. In the multi-edge Graph, edges $e_{ij}$ are typically constructed based on the Euclidean distance $d_{ij}$ between atoms $v_i$ and $v_j$. For
$d_{ij}=||\boldsymbol{p}_{j}+k_{1}\boldsymbol{l}_{1}+k_{2}\boldsymbol{l}_{2}+k_{3}\boldsymbol{l}_{3}-\boldsymbol{p}_{i}||_{2}\leq R$,
when the Euclidean distance $d_{ij}$ between atoms $v_i$ and $v_j$ is less than a given radius $R$, an edge $e_{ij}$ with the initial edge feature $d_{ij}$ is created between $v_i$ and $v_j$. 
Different values of $\boldsymbol{k}=[k_{1},k_{2},k_{3}]\in\mathbb{R}^{3}$ represent different edges between nodes $v_i$ and $v_j$.
After constructing the crystal graph,
CGCNN builds a CNN on top of the crystal graph, using convolution and pooling layers to extract and learn local and global features of the crystal structure. These convolution and pooling layers also achieve invariance to atomic indexing and unit cell selection. 
Additionally, by separating the convolution and pooling layers, CGCNN can learn the contributions of different local chemical environments to the target properties, thus providing interpretable prediction of properties.







%CFID~\cite{choudhary2018machine} 
Although CGCNN has achieved impressive results, there is still much room for improvement. For example, CGCNN lacks a description of global states (such as temperature), which is necessary for predicting state-dependent properties (such as free energy). MEGNet~\cite{chen2019graph} improves the CGCNN model by introducing global state inputs, including temperature, pressure, and entropy. During the updates of bond embeddings and node embeddings, the embeddings of global state information are also updated simultaneously. 
The CGCNN model focuses only on capturing local atomic environments, while GATGNN \cite{louis2020graph} combines augmented graph attention layers and global attention layers to focus on the different contributions of various atoms in a crystal to the overall material properties. 
The augmented graph attention layer aggregates information from neighboring nodes by calculating attention weights between nodes, while the global attention layer operates on the graph's overall structure.
In contrast to the these typical GNN architectures like CGCNN, MEGNet, and GATGNN,
ALIGNN employs a line graph neural network, which is derived from a crystal graph~\cite{choudhary2021atomistic,kaundinya2022prediction}. This derived graph describes the connectivity of the edges in the original crystal graph, with its nodes corresponding to atomic bonds and its edges representing bond angles. ALIGNN alternates message passing on these two graphs, leveraging bond lengths and angles in the line graph to incorporate detailed atomic structural information, thereby improving the model's performance.








%\begin{comment}
    
\begin{figure}[t!] 
  \centering   
  \includegraphics[width=6.8in]{fig/overview-property-gnn_new22.pdf}
  \caption{\textbf{GNN-based methods for property prediction.} 
  \textbf{a $|$} Schematic of CGCNN method. This model first represents crystal structures as multi-edge graphs and then uses graph convolutional neural networks to process them. 
  \textbf{b $|$} CGCNN experimental results: The top shows a line chart of MAE loss using different graph convolution functions, and the bottom is a 2D histogram representing the predicted formation energy per atom against the DFT calculated value.
  \textbf{c $|$} The CrysGNN method uses a large number of unlabeled crystal graphs during the pre-training phase to learn structural and chemical information. Then, the pre-trained CrysGNN model is retrofitted into any SOTA property predictor to enhance its learning process and improve performance. In the experimental results at the bottom, the green bars represent the final improved MAE results.
  Panel \textbf{a} and \textbf{b} adapted from REF.~\cite{xie2018crystal}. Panel \textbf{c} adapted from REF.~\cite{kaba2022equivariant}.
 }
  \label{fig:overview-property}
\end{figure}
%\end{comment}



Compared to molecules, crystals typically exhibit higher structural symmetry, a feature often overlooked by previous models. 
Kaba et al. \cite{kaba2022equivariant} developed an equivariant model for crystal symmetry groups. Due to the fact that crystal space groups are usually much smaller than symmetry groups, equivariance to smaller groups results in less constrained parameter sharing and more expressive models. 
CrysGNN \cite{das2023crysgnn}, unlike traditional end-to-end supervised learning approaches that directly use GNNs, is a pre-training framework for GNNs. In the pre-training stage of CrysGNN, it reconstructs node features and connectivity in a self-supervised manner. Meanwhile, it leverages the space group and crystal system information of crystal materials to learn structural similarities between graph structures. 
This training paradigm enables CrysGNN to utilize the latent chemical and structural information present in a large amount of unlabeled crystal data, which can then be used to distill the property predictor, improving the accuracy of property prediction.


Compared to aforesaid GNN-based methods for predicting crystal properties, which construct graphs by creating edges between atoms within a predetermined distance threshold, 
PotNet \cite{lin2023efficient} directly models the interatomic potentials as edge features to capture the interactions between atoms in infinite space. Additionally, it models the complete potential set between all atoms through the approximation of infinite potentials, rather than only modeling between nearby atoms as previous methods did, resulting in improved performance.



Traditional invariant GNNs are incompatible with directional properties, which limits their current applications to predicting invariant scalar properties and makes them difficult to apply to predicting tensor properties of crystals (such as dielectric tensors). In contrast, 
The Edge-based Tensor Prediction Graph Neural Network (ETGNN)~\cite{zhong2023general} represents a crystal's tensor properties as the average of the tensor contributions from all atoms in the crystal. Each atom's tensor contribution can be expressed as a linear combination of local spatial components projected onto the directions of edges of multiple-sized clusters. This tensor decomposition is rotationally equivariant, allowing it to be applied to the prediction of tensor properties.
GMTNet~\cite{yan2024space} is designed for predicting general tensor properties of crystalline materials, including dielectric tensors, piezoelectric tensors, and elastic tensors. Within the broad framework of GNNs, GMTNet adopts the transformer strategy from Comformer \cite{yan2024complete} to update node invariant features. It then employs spherical harmonic filters and tensor product convolutions to achieve equivariant message passing, updating edge features.
In addition to achieving tensor equivariance and adhering to crystal symmetry constraints, GMTNet incorporates an additional crystal symmetry enforcement module. 
This module simplifies the complex symmetry constraints of tensor properties into constraints applicable to crystal-level features, further constraining the network's output. This design also provides robustness against minor errors in the message-passing operations and crystal inputs.



Currently, the predominant approach for predicting the properties of crystalline materials is supervised learning. In this approach, substantial time is often required to train models that map input crystal data to their corresponding properties. To overcome this challenge, Song et al. \cite{song2024diffusion} proposed a pretrain-fnetune framework named CrysDiff for crystal property prediction tasks based on a diffusion model. CrysDiff consists of two stages: pre-training and fine-tuning. In the pre-training stage, similar to other diffusion models in crystal generation tasks \cite{jiao2023crystaliclr}, CrysDiff learns the latent marginal distribution of crystal structures. In the fine-tuning stage, while keeping the input crystal structure unchanged, CrysDiff learns the distribution of crystal properties. The fine-tuning stage only trains MLP responsible for outputting crystal properties. %The pre-training stage enables CrysDiff to learn to recognize important patterns within crystal structures, which accelerates the learning process in the fine-tuning stage.


\subsubsection{String-Based Prediction}
Transformers first appeared in research within the field of NLP \cite{vaswani2017attention}. Due to their powerful representation capability of the self-attention mechanism and the ability to process sequences in parallel, 
they can naturally be applied to the field of crystal material research. 
When specifically applying the Transformer network structure, it is common to first perform embedding encoding on the node and edge features of the crystal graph. 
For node features, GNNs are used for embedding encoding, such as using CGCNN~\cite{xie2018crystal} for node feature encoding in REF. \cite{yan2024complete, yan2022periodic}. For edge features, radial basis function (RBF)~\cite{choudhary2021atomistic} is typically employed.


Matformer \cite{yan2022periodic} is a periodic invariant transformer-based network. It introduces a novel approach for representing periodic graphs by utilizing the geometric distances between identical atoms in adjacent unit cells (represented as self-connecting edges in the graph) to encode periodic patterns. 
By combining these geometric distances with lattice parameters, Matformer effectively captures the lattice size and periodic pattern information of a given crystal in an implicit manner.
By directly encoding periodic patterns using self-connecting edges, Matformer can effectively represent the periodic structure of crystals. However, Matformer sometimes encodes crystals with different structures as the same graph \cite{yan2024complete}. ComFormer \cite{yan2024complete} circumvents this issue. It
proposed SE(3) invariant representation (using atomic interatomic distance and relative atomic angle information to represent edge features of the graph) and SO(3) equivariant crystal graph representation (using atomic interatomic distance vector form to represent edge features of the graph), effectively capturing the complete geometric information of infinite crystals. Then, ComFormer converts these two types of crystal graphs into embeddings and utilizes the transformer structure, including Node-wise transformer layer and Edge-wise transformer layer, to express expressive geometric information in message passing.
Compared to Matformer, which only focuses on geometric information between atoms, CrystalFormer~\cite{wang2024conformal} also retains angular data. It introduces a robust graph construction method specifically designed for periodic invariance, using different penalty weights to select appropriate atomic neighborhoods, effectively distinguishing crystals. Additionally, CrystalFormer enhances long-range information by incorporating an angular attention mechanism.




Since crystal structures exhibit infinite repetition, incorporating the attention mechanism with infinite connectivity between atoms is necessary when using the Transformer architecture. Conventional models like Matformer often neglect the influence of distant atoms during processing, but 
Crystalformer~\cite{taniai2024crystalformer} interprets the infinite connectivity attention as a physically inspired infinite summation of interatomic potentials in an abstract feature space. This approach effectively incorporates long-range atomic interactions, where the infinite connectivity approximation becomes tractable due to the exponential decay of interatomic distances. 
%The network architecture of Crystalformer is similar to the original Transformer encoder architecture \cite{}, featuring stacked self-attention blocks while removing the normalization layer.


%Wang et al. \cite{wang2024conformal} introduces a robust graph construction method specifically designed for periodic invariance. Building upon a k-connected graph foundation, this method utilizes different penalty weights to select suitable neighborhoods for atoms, effectively reducing the randomness of physical properties. Additionally, the paper presents a transformer architecture called CrystalFormer(AAAI) that emphasizes angle preservation and enhances long-range information by incorporating an angle attention mechanism. When embedding edge features of the graph data, CrystalFormer(AAAI) employs a method based on Dirichlet energy minimization and harmonic mapping, approximating a neural network's conformal mapping to preserve the intrinsic angle information in the crystal graph. %Furthermore, the architecture incorporates an angle attention mechanism that further enhances both angle preservation and long-range information.



DOSTransformer \cite{lee2024density} is a method specifically designed for density of states prediction (DOS). Since DOS is not only determined by the material itself but also by the energy levels considered during DOS calculation, DOSTransformer takes both the crystal material and energy as heterogeneous input modalities. After obtaining the atomic embedding, DOSTransformer utilizes cross-attention layers and self-attention layers of the multi-modal transformer to capture the relationships between the crystal material and various energy levels. Additionally, DOSTransformer provides additional structural information about the crystal material to the self-attention layers through learnable prompts.




Unlike the prediction of other single-valued properties of crystals, adsorption energy describes the energy change when one substance (such as gas molecules) adsorbs onto another substance (such as the surface of a crystalline material). Therefore, when using ML methods to predict adsorption energy, the model inputs often involve both the adsorbent and the adsorbate, i.e., the crystal and the molecule. In previous work, GAME-Net \cite{pablo2023fast}  constructed a graph based on adsorption systems, taking the molecule and the atoms on the crystal surface it binds to as an atomic system input, using graph neural networks for adsorption energy prediction. AdsorbML \cite{lan2023adsorbml} took the crystal surface of the molecule as an atomic system input, using machine learning methods to find the lowest energy adsorption systems and then using DFT to predict the adsorption energy.
Uni-MOF~\cite{wang2024comprehensive} is a more comprehensive transformer-based adsorption property prediction framework that primarily focuses on predicting the gas adsorption properties of crystalline porous materials, i.e. MOF (metal-organic frameworks) materials. This framework pre-trains on large-scale MOF and COF (covalent organic frameworks) structures and subsequently fine-tunes and predicts with inputs such as MOF materials, gas molecules, temperature, and pressure. During pre-training, Uni-MOF uses a large-scale dataset of MOFs and COFs to perform masked atom prediction and introduces noise into the original coordinates of MOFs before coordinates reconstruction. This approach promotes a deeper understanding of the material's spatial structure in the pre-trained model, enhancing its robustness and generalization. The fine-tuning process involves training the model under various adsorption conditions, enabling the fine-tuned Uni-MOF to predict multi-system adsorption properties of MOFs under any state (including different gases, temperatures, and pressures).

% \subsubsection{Diffusion-Based Methods}






%\begin{comment}
\begin{figure}[t!] 
  \centering   
  \includegraphics[width=6.8in]{fig/overview-property-transformer_new2.pdf}
  \caption{\textbf{Schematic overview of Uni-MOF framework.} 
  \textbf{a $|$} In the pre-training phase, in addition to predicting the types of occluded atoms, a three-dimensional position denoising task is used to learn three-dimensional spatial representations. Cross-system performance datasets can be collected or randomly sampled under different operating conditions. During the fine-tuning phase, a unified gas adsorption prediction model, Uni-MOF, is established by embedding pre-trained weights, MOF materials, gas, temperature, and pressure.
  \textbf{b $|$} 
  Uni-MOF experimental results:
  adsorption isotherms based on low-pressure predictions and highpressure experimental values.
  Panel \textbf{a} and \textbf{b} adapted from REF.~\cite{wang2024comprehensive}. 
 }
  \label{fig:overview-property}
\end{figure}
%\end{comment}


\subsection{Crystalline Material Synthesis}





Traditionally, the discovery of novel crystalline compounds has relied heavily on intuition, trial-and-error experimentation, and serendipity. However, the chemical space of possible crystalline structures is immense, making it infeasible to exhaustively explore through physical synthesis and characterization alone. In recent years, deep generative models such as GANs, VAEs, diffusion, flow matching\cite{chen2018neural}, Transformer, etc, have offered a promising new avenue for accelerating crystalline material discovery. By learning from large datasets, they have shown the potential to learn the underlying patterns and rules governing the structure-property relationships of crystalline materials. According to data representation, existing methods fall into two categories: geometric graph-based generation and text-based generation. Based on this taxonomy, Table \ref{tab:generation} provides a brief summary of the used data representations, backbone models, physical priors, and whether the model can achieve guided generation of target properties.


\subsubsection{Geometric Graph-Based Generation}



% Traditionally, material discovery has largely depended on experimental exploration and human intuition, which entail extensive computational and time costs.
% One of the key challenges in novel materials generation lies in characterizing the structural relationships between atoms. As the number of atoms increases, the inter-atomic relationships become increasingly complex, which prevents traditional experimental methods from scaling effectively to large materials with intricate inter-atomic relationships. 

% Deep generative models, such as VAE, GANs, diffusion models, language models, etc, have shown potential for modeling scientific data, including small molecules, proteins, and their complexes. To scale these deep generative models to materials, recent works designed deep generative models to automatically discover inter-atomic relationships in data to generate novel materials.

% Typically, existing studies incorporated physical priors or constraints into the models to explicitly or implicitly model the complex atomic systems of materials. Among others, a number of studies generate materials from scratch without conditions. Towards generating materials with specific structures or properties, the most recent works leveraged structural information or properties as conditions for controllable or conditional generation. 


%  the most recent works incorporated physical priors or constraints into the models for conditional generation. Furthermore, some studies leverage physical properties as conditions to generate materials with target properties for controllable generation. 

% ensure the periodicity, symmetry, and structure validity, thus explicitly modeling complex atomic systems of crystal materials. 



\begin{table*}[!h]\small
  \centering
  \caption{Summary of Deep Generative Models for Material Generation}
    \rowcolors{2}{gray!25}{white}
\renewcommand\arraystretch{1.35}
    \begin{tabular}{lllll}
    \toprule
    Methods & Data representation & Base models & Physical knowledge/constraints & Guided generation \\
    \midrule
     G-SchNet~\cite{gebauer2019symmetry} & Cartesian coordinate  &  Geometric GNNs & Symmetry& Scalar property\\
     % FTCP~\cite{ren2020inversegeneralized}  & Cartesian Coordinate &  VAE &  & \\
    CDVAE~\cite{xie2021crystal} & Cartesian coordinate & Diffusion & Harmonic approximation & Scalar property\\
Con-CDVAE\cite{ye2024concdvae} & Cartesian coordinate & Diffusion & Property constraints & Scalar property\\
Cond-CDVAE\cite{luo2024deep} & Cartesian coordinate & Diffusion & Property constraints & Scalar property\\
     LCOMs~\cite{qi2023latent}& Cartesian coordinate  & Diffusion &  Property constraints & Scalar property \\ 
         DiffCSP~\cite{jiao2023crystal} & Fractional coordinate & Diffusion & Symmetry constraint & Structure property\\
EquiCSP~\cite{linequivariant }& Fractional coordinate & Diffusion & Symmetry & -\\
         
GemsDiff~\cite{Klipfel_Fregier_Sayede_Bouraoui_2024}& Cartesian coordinate  & Diffusion &  Composition constraint& -\\ 
       SyMat~\cite{luo2024towardssymmetry} & Cartesian coordinate & Diffusion & Symmetry & Scalar property\\
            EMPNN~\cite{klipfel2024equivariant}& Cartesian coordinate  & Geometric GNNs &  Group actions &-\\ 
            UniMat~\cite{yang2023scalable} &  
 Cartesian coordinate &  Diffusion & -& Both
\\    MatterGen~\cite{zeni2023mattergen}& Cartesian coordinate  & Diffusion & Property constraints & Composition property \\ 
    PGCGM~\cite{zhao2023physics}& Fractional coordinate  & GAN &  Atomic distance and symmetry& Structure property\\ 
CubicGAN~\cite{zhao2021highcubiccrystal}& Fractional coordinate  & GAN &  Space group& Structure property\\ 
    PCVAE~\cite{10191051}& Cartesian coordinate  & VAE &  Space group& Structure property\\ 
       DiffCSP++~\cite{jiao2024space} & Fractional coordinate & Diffusion & Space group: Wyckoff position & Structure property\\
       FlowMM\cite{miller2024flowmm}& Fractional coordinate & Flow matching & Periodic lattice  &Composition property\\
      % PGD-VAE~\cite{wang2022deep}& Cartesian Coordinate  & VAE & unit cells to guarantee periodicity& \\ 
Govindarajan~\cite{govindarajan2023behavioral,govindarajan2023learning}  & Cartesian coordinate  & Geometric GNNs   & -& Structure property \\
   CHGFlowNet ~\cite{nguyen2023hierarchical}  & Cartesian coordinate  & Geometric GNNs   & Space group & Structure property \\
         LM-CM,LM-AC~\cite{flam2023language} & Text-CIFs  & GPT architecture &  - & Structure property\\ 
         CrystaLLM~\cite{antunes2023crystal} & Text-CIFs  & GPT architecture  &  - & Both\\ 
    CrystalFormer~\cite{cao2024space}& Text-CIFs  & Transformer &  Space group: Wyckoff position & Structure property \\ 
    SLI2Cry~\cite{xiao2023invertible} & Text-SLICES & RNN   &  Force field & Structure property\\
Gruver~\cite{gruver2024finetuned} &  Text-CIFs & LLaMA-2 & -& Both\\
    \bottomrule
    \end{tabular}%
  \label{tab:generation}%
\end{table*}%

% \subsubsection{Unconditional Generation}

Crystalline materials can be naturally represented as geometric graphs in the Euclidean space. Generally, the geometric graphs are represented in two coordinate systems, i.e., the Cartesian coordinate system and the fractional coordinate system. Early work seldom considered equivariance and invariance to permutation, rotation, translation, and periodic transformations~\cite{ren2020inversegeneralized,court3d20203}, suffering from low validity of generated materials~\cite{xie2021crystal}.
Due to the bedrock of geometric GNNs in modeling geometry, geometric graphs-based generative models typically use geometric GNNs to ensure equivariance and invariance of the generated materials~\cite{batatia2022mace,schutt2021equivariant,vignac2020building,klipfel2024equivariant}.

 % play the bedrock  to ensure the equivariance and invariance to permutation, rotation, translation, and periodic transformations. Therefore, such as the symmetry constraints of translations, rotations, and/or reflections of materials. 

%They transform 3D graph representation into distance/angle/dihedral-based scalars that are invariant to rotations or translation and recover the directional information of the processed scalars for preserving equivariance.

One pioneer is G-SchNet~\cite{gebauer2019symmetry}. G-SchNet incorporates the constraints of Euclidean space and the rotational invariances of the atom distribution as prior knowledge. By using the distance between the previously placed positions and the next atomic position as constraints, an equivariant conditional probability distribution is constructed to determine the next atomic position. FTCP~\cite{ren2020inversegeneralized} is a crystal representation that concatenates real-space properties (atom positions, atom types, etc.) and Fourier-transformed momentum-space properties (diffraction pattern). A 1D CNN-VAE is trained over this representation for crystal generation. 





By using the SE(3) equivariant message-passing neural networks as the encoder and decoder, CDVAE~\cite{xie2021crystal} explicitly encodes the geometry graph and its lattice as invariant variables for permutation, translation, rotation, and periodic invariances. Conditioning on these invariant variables, CDVAE generates materials in a diffusion process that moves atomic coordinates towards a lower energy state and updates atom types to satisfy bonding preferences between neighbors. In addition, CDVAE shows the ability to generate materials with specific properties. CDVAE jointly trains a property predictor to predict properties of training materials from latent $z$. To optimize properties, CDVAE starts with the latent representations of testing materials and applies gradient ascent in the latent space to improve the predicted property.



\begin{figure}[!h] 
  \centering   
  \includegraphics[width=6.3in]{fig/generation.pdf}
  \caption{} 
  \label{fig:overview-generation}
\end{figure}
%\end{comment}









%%%%%%%%%%%%%% periodical+lattice para+stable
% Xie \textit{et al.} adopts an equivariant variational auto-encoder-based framework, called CDVAE, to learn the data distribution and then generates crystals in a score-matching-based diffusion process. 

Based on the CDVEA, researchers have made several extensions. Cond-CDVEA\cite{luo2024deep} extends CDVAE to be capable of generating valid, diverse crystal structures conditioned on user-defined chemical composition and pressure. Similarly, Con-CDVEA\cite{ye2024concdvae} generates crystals’ latent variables according to given properties (e.g., formation energy, band gap, crystal system, combination of formation energy and band gap) and then yields the corresponding crystal structure by decoding the latent variables.
Towards generating stable crystal structure, LCOMs~\cite{qi2023latent} expanded on CDVAE to explore and identify the crystal structure with the lowest energy corresponding to a specific chemical formula. LCOMs transform crystal structures into latent representations, following which gradient-based optimization techniques are applied within this latent space to locate the structures with the lowest energy.

 % Subsequently, the optimized latent vector, associated with the lowest predicted energy, is decoded to yield the corresponding crystal structure.
%%%%%%%%%%%%%% periodical+lattice para+lowest predicted energy


Unlike CDVAE, which uses the Cartesian system, DiffCSP~\cite{NEURIPS2023_38b787fc} utilizes the fractional coordinate system to intrinsically represent crystals and model periodicity. In particular, by employing an equivariant graph neural network for the denoising process, DiffCSP~\cite{NEURIPS2023_38b787fc} introduced an equivariant diffusion approach, which conducts joint diffusion on lattices and fractional coordinates to comprehensively capture the crystal geometry, thereby enhancing the modeling of the crystal geometry. Theoretically, it has been demonstrated to generate periodic-E(3)-invariant samples. However, DiffCSP does not generate atom types of periodic materials, but lattices and atom coordinates from the input atom types, so DiffCSP cannot be applied to design novel periodic materials from scratch. Similar to DiffCSP, GemsDiff~\cite{Klipfel_Fregier_Sayede_Bouraoui_2024} employs an equivariant graph neural network and jointly considers atomic positions and crystal lattices. It applies a diffusion process to both atomic positions and crystal lattices to learn the structural geometry.


SyMat~\cite{luo2024towardssymmetry} aims to capture physical symmetries of periodic material structures. A score-based diffusion model uses periodic invariant multi-graph representations of materials as inputs to generate atom coordinates and it calculates coordinate matrix from the edge distance score functions to ensure invariance to all symmetry transformations. SyMat achieves invariance to physical symmetry transformations of periodic materials, including permutation, rotation, translation, and periodic transformations. Following CDVAE's manner, SyMat can also generate materials with a specific property. 
EMPNN~\cite{klipfel2024equivariant} enforces a structuring bias adapted to crystals using group actions incorporated by the equivariance property of MPNN layers. The work generalizes the interaction force between atoms to any orientation. By taking advantage of this property, the equivariant representation enhances the generalization capability of the crystal lattice.
%%%%%%%%%%%%%% SL3(Z)?????

%%%%%%%%%%%%%% gradually refining atom types, coordinates, and the periodic lattice ， 
Zeni \textit{et al.}~\cite{zeni2023mattergen} present MatterGen, a model that generates stable, diverse inorganic materials across the periodic table. To enable this, MatterGen uses a diffusion-based generative process that produces crystalline structures by gradually refining atom types, coordinates, and the periodic lattice. In particular, an equivariant score network is pre-trained on a large dataset of stable material structures to jointly denoise atom types, coordinates, and the lattice. The score network is then fine-tuned with a labeled dataset, where the property labels are encoded to steer the generation towards a broad range of property constraints, such as desired chemistry, symmetry, and scalar property constraints.
%%%new  representation scalability    a unified crystal representation that can represent any crystal structure
UniMat~\cite{yang2023scalable} developed a periodic table-based material representation to model represent material with a finite number of atoms in a unit cell. UniMat defined a 4-dimensional material space $R^{L\times H\times W\times C}$. where $H$ = 9 and $W$ = 18 corresponds to the number of periods and groups in the periodic table, $L$ corresponds to the maximum number of atoms per element in the periodic table, and $C$ = 3 corresponds to the $x,y,z$ locations of each atom in a unit cell. The representation shows flexibility for smaller systems, as one can set $H$ and $W$ to model specific chemical systems of interest. For example, set $H$ = 1, $W$ = 1 for modeling materials containing one specific element. With such a unified representation of materials, UniMat trains diffusion models by treating the representation as a 4-dimensional tensor input or condition.

Despite the success of the above methods, one significant aspect that has been largely overlooked is the consideration of space group symmetry. Space groups play a pivotal role in crystallography, defining the geometry of crystal structures and being intrinsically tied to many properties, such as the topological phases. 
Zhao \textit{et. al.} proposed a GAN model, called CubicGAN~\cite{zhao2021highcubiccrystal}, to generate large-scale cubic materials conditioning on the elements and a specified space group. Furthermore, Zhao \textit{et. al.}~\cite{zhao2023physics} also proposed PGCGM, a physics-guided deep learning model for the generative design of crystal materials with high symmetry. Conditioning on element constituents and space groups, PGCGM devises two physics-oriented losses based on atomic pairwise distance constraints and structural symmetry into the generative adversarial network, thus generating crystal materials with high symmetry. However, the application of PGCGM is constrained by ternary systems, thus limiting its universality. Besides, PCVAE~\cite{10191051} integrates space group constraints to predict lattice parameters using a conditional VAE.

DiffCSP++~\cite{jiao2023space} further interpret the space group constraint into two tractable parts: the basis constraint of the O(3)-invariant logarithmic space of the lattice matrix and the Wyckoff position constraint of the fractional coordinates. DiffCSP++ separately and simultaneously generates the lattices, fractional coordinates, and atom composition under the reduced form of the space group constraint. Upon the derived constraints, DiffCSP++ enables structure generation under given space group constraints, hence allowing the creation of diverse structures from the same composition but based on different space groups.
EquiCSP \cite{linequivariant} addresses the challenge of lattice permutation equivariance in diffusion models by incorporating a permutation invariance penalty term during the denoising model training. Additionally, EquiCSP introduces a novel diffusion noising method known as Periodic CoM-free Noising, which maps all equivalent periodic data to the same representation and addresses periodic translation invariance. This approach enables the Score-Matching method in SDEs to achieve periodic translation equivariance in crystal generation. Compared to the DiffCSP method, EquiCSP fully realizes E(3) equivariance based on periodic graph symmetry during the diffusion training process.

FlowMM \cite{miller2024flowmm} generalizes the Riemannian flow matching for estimating a point cloud density to the material domain to ensure invariances. Specifically, FlowMM focuses on crystal structure prediction, i.e., predicting the stable crystal structure of a known composition of elements, and De Novo generation, i.e., finding novel compositions along with their stable structures. Compared to diffusion models, FlowMM is able to generate materials with comparable stability to these other methods while being significantly faster at inference time

Some work uses reinforcement learning methods to autoregressively generate materials. Govindarajan~\cite{govindarajan2023behavioral,govindarajan2023learning} formulates the problem of designing new crystals as a sequential prediction task. At each step, given an incomplete graph of a crystal skeleton, an agent assigns an element to a specific node. The policy network is a graph neural network that transforms a given state into an effective representation and predicts the action. Similarly, CHGFlowNet ~\cite{nguyen2023hierarchical} used a graph neural network-based hierarchical policy network to generate materials, where high-level decision-making policy operates on the space groups, and the low-level execution policy operates on the atom-lattices policy actions. 
%%%%%%%%%%%%%% space groups



% Unconditional generation cannot control the generation process to generate materials with desirable structures or properties. They mainly focus on incorporating physical knowledge toward generating valid and stable materials. In particular, because crystalline materials can be represented as 3D point data or string data, considerable endeavors incorporate physical knowledge into the deep generative models from computer vision and natural language processing domains, such as VAEs, GANs, diffusion models, graph neural networks, Transformer, etc. In the following paragraphs, we summarize the existing unconditional generation methods.

% \textbf{Graph representation.}

% \textbf{3D representation.}




% Gebauer \textit{et. al.}~\cite{gebauer2019symmetry} developed the autoregressive G-SchNet for molecule generation of rotationally invariant 3d point sets. In contrast to generative networks on point cloud generation, G-SchNet 



 
%%%%%%%%%%%%%% lattices and fractional coordinates





% In contrast to CDVAE, which predicts the lattice and then updates the coordinates with a fixed lattice, DiffCSP~\cite{NEURIPS2023_38b787fc} 





% Since CDVAE, several works have extended diffusion processes to capture all parameters of the crystal, not just the atomic coordinates.

 
%MPNNs allow the processing of sparse data and can be designed to be invariant or equivariant to many group actions.





% By regarding the material's unit cells as local patterns and the connections of unit cells as global patterns, Wang \textit{et. al.}~\cite{wang2022deep} developed a deep generative model called PGD-VAE, including a global-pattern encoder, a local-pattern encoder, a local structure decoder, a neighborhood decoder, and a global structure decoder to guarantee periodicity. By regarding the material's unit cells as local patterns and the connections of unit cells as global patterns, PGD-VAE shows the ability to model periodical materials such as metal-organic materials.

% disentanglement of the local and global patterns by ensuring the invariance of the local patterns

%%%%%%%%%%%%%% periodical



% \textbf{1D representation.}

% Graph representation of materials can represent the local environment of each atom and structure periodicity. Recent works suggested using Graph Neural Networks for materials. MPNNs allow the processing of sparse data and can be designed to be invariant or equivariant to many group actions. Most of the existing works are equivariant to SO(3). Thanks to a spherical basis that allows us to predict lattice properties and perform simulations. However, these methods are not able to deform crystal lattices where the shape of the lattice is unknown in advance. In addition, these works are equivariant to subgroups of the Euclidian group but do not consider other group actions such as SL3(Z).



% \subsubsection{Conditional Generation}

%可以特定结构

% Conditional generation not only aims to generate stable and valid materials but also needs to produce materials with specific structures or properties.



%Despite the promising performance, generative adversarial networks are notoriously hard to train because of saturation and mode collapse in discriminator.

\subsubsection{String-Based Generation}

Crystals are stored in standard text file formats known as CIFs, i.e., Crystallographic Information Files. Within CIFs, the structural information necessary to describe the crystal includes atomic elements and coordinates as well as the parameters defining the periodic lattice. CIF files include atomic elements positioned in a unit cell or lattice, with six additional parameters necessary to define the unit cell. By treating CIFs as plain text, some work explore the use of language models to generate crystals. In addition, invertible and invariant crystal representation, SLICES, also promotes the use of language models in material generation.


%%%%% cif as text
Flam-Shepherd \textit{et al.}~\cite{flam2023language} uses sequences of discrete tokens to represent everything, including the digits of atomic coordinates. With all data encoded as tokens, standard language modeling methods designed for text can be applied with little to no modification. The simplicity of this method also makes it simple to adapt to many different kinds of molecular structures, including small molecules, protein binding pockets, and, of course, crystals. The work demonstrates that language models trained from scratch on many common molecular datasets actually outperform popular domain-specific models in their ability to generate valid compositions and structures. Similarly, Antunes \textit{et al.}~\cite{antunes2023crystal} also developed a language model called CrystaLLM to generate crystal structures as discrete sequences by training from scratch on millions of CIF strings. Particularly, the integration with predictors of formation energy permits the use of a Monte Carlo Tree search algorithm to improve the generation of structures with lower formation energy.

%space group symmetry  Wyckoff
Cao \textit{et al.}~\cite{cao2024space} introduces CrystalFormer, a transformer-based autoregressive model specifically designed for space group-controlled generation of crystalline materials. The space group symmetry significantly simplifies the crystal space, which is crucial for data and computing efficient generative modeling of crystalline materials. In CrystalFormer, the crystalline materials are represented by the Wyckoff letter, chemical elements, and fractional coordinates, and a transformed conduct mask learning by masking the Wyckoff letter, chemical element, and fractional coordinates. To generate new samples, the transformer sequentially samples atom types, coordinates, Wyckoff positions, and lattice parameters.
Gruver \textit{et. al.}~\cite{gruver2024finetuned} showed that fine-tuned LLMs can generate the three-dimensional structure of stable crystals as text. The work converts the crystal lattice, atom identities, and atom positions into strings, and LLaMA-2 models are fine-tuned on the strings of inorganic materials. By using string formatted crystals and task-specific prompting, the work enables unconditional stable materials generation, text-condition materials generation, and structural infilling. 

Based on the SLICES representation, SLI2Cry\textit{et al.}~\cite{xiao2023invertible} applies SLICES for the inverse design of direct narrow-gap semiconductors for optoelectronic applications. Firstly, a general recurrent neural network was trained on the Materials Project database to learn the syntax of SLICES strings and fine-tuned on a dataset of direct narrow-gap semiconductors. The fine-tuned RNN was used to generate large volumes of SLICES strings, which were then reconstructed into crystal structures using the SLICES decoding. Specifically, a desired formation energy can be input into the model to sample strings. By repairing the strings to generate valid SLICES strings, corresponding crystals can be reconstructed.



% Apart from generating materials with specific structures, some works explore generating materials with property constraints.


% \subsubsection{Controllable Generation}

%可以特定属性

% Despite the progress in graph neural networks for general graphs, they cannot be directly applied to handle materials with periodicity.




% Motivated by non-equilibrium thermodynamics, diffusion models connect the data distribution with the prior distribution via forward and backward Markov chains and have made remarkable progress in the field of image generation. Equipped with equivariant GNNs, diffusion models are capable of generating samples from the invariant distribution, which is desirable in conformation generation, molecule design, protein generation, and crystal material design.

% Typically, these diffusion models were designed with a careful eye towards symmetries and are built on top of graph neural networks with strict invariance/equivariance properties.










\subsection{Aiding Characterization}

\subsubsection{Image-Based Aiding Characterization}

The atomistic images obtained by microscopy techniques encompass a broad range, from resolving local atomic structures to mesoscale morphologies (microstructure), unveiling the distribution and types of defects, as well as their dynamics. This data is intimately connected to the materials' functionality and performance, underscoring the importance of microscopic examination in understanding and optimizing material properties. With the atomistic images, a broad portfolio of image-based material characterization techniques has been proposed. In this part, we briefly introduce these image-based characterization techniques.

One of the characterization techniques is to generate predictions for every pixel in an image, furnishing a wealth of detailed information about the size, position, orientation, and morphology of features of interest. Notably, Azimi et al.~\cite{azimi2018advanced} developed an ensemble of fully convolutional neural networks to accurately segment martensite, tempered martensite, bainite, and pearlite in scanning electron microscopy (SEM) images of carbon steels, achieving a remarkable accuracy of 94\%. Their methodology represents a significant advancement over previous attempts to automate the segmentation of different phases in SEM images, underscoring the efficacy of deep learning in materials characterization. Modarres et al. applied transfer learning to automatically classify SEM images of different material systems~\cite{modarres2017neural}. They demonstrated how a single approach can be used to identify a wide variety of features and material systems, such as particles and fibers.


% DL can be applied to generate one or more predictions for every pixel in an image. This can provide more detailed information about the size, position, orientation, and morphology of features of interest in images. Thus, pixelwise learning has been a significant area of focus with many recent studies appearing in materials science literature. Azimi et al. applied an ensemble of fully convolutional neural networks to segment martensite, tempered martensite, bainite, and pearlite in SEM images of carbon steels. Their model achieved 94\% accuracy, demonstrating a significant improvement over previous efforts to automate the segmentation of different phases in SEM images. 


Deep learning has been effectively utilized to identify the symmetries present in simulated measurement data of materials. Ziletti \textit{et al.} ~\cite{ziletti2018insightful} paved the way for this application by creating a large database of perfect crystal structures, purposefully introducing defects into these ideal lattices, and subsequently simulating diffraction patterns for each structure. By training deep learning models to classify the space group of each diffraction pattern, the researchers achieved remarkable performance, even in the presence of significant defects. Notably, the deep learning model outperformed traditional algorithms in detecting symmetries from diffraction patterns, highlighting the potential of deep learning to augment our understanding of materials at the atomic scale.

% Deep learning has also been applied to characterize the symmetries of simulated measurements of samples. Ziletti et al.~\cite{ziletti2018insightful} obtained a large database of perfect crystal structures, introduced defects into the perfect lattices, and simulated diffraction patterns for each structure. DL models were trained to identify the space group of each diffraction pattern. The model achieved high classification performance, even on crystals with significant numbers of defects, surpassing the performance of conventional algorithms for detecting symmetries from diffraction patterns.


Distinguishing individual instances of recognized objects within an image is crucial, requiring object detection or localization. When instances barely overlap, post-processing of semantic segmentation outputs can be employed to resolve these individual instances. This approach has been extensively applied to identify individual atoms and defects in microstructural images. A notable example is provided by Yang et al.\cite{yang2021deep}, who utilized the U-net architecture to attain high accuracy in detecting vacancies and dopants in WSe2 STEM images, achieving a model accuracy of up to 98\%. To classify these atomic sites, they grounded their approach in experimental observations, categorizing the sites into five distinct types: tungsten, vanadium replacing tungsten, selenium with no vacancy, monovacancy of selenium, and divacancy of selenium.

% Object detection or localization is needed when individual instances of recognized objects in a given image need to be distinguished from each other. In cases where instances do not overlap each other by a significant amount, individual instances can be resolved through post-processing of semantic segmentation outputs. This technique has been applied extensively to detect individual atoms and defects in microstructural images. For example, Similarly, Yang et al.\cite{yang2021deep} used U-net architecture to detect vacancies and dopants in WSe2 in STEM images with model accuracy of up to 98\%. They classified the possible atomic sites based on experimental observations into five different types: tungsten, vanadium substituting for tungsten, selenium with no vacancy, mono-vacancy of selenium, and di-vacancy of selenium.


% \subsection{Spectra Prediction}



\subsubsection{Spectra-Based Aiding Characterization}


When electromagnetic radiation hits materials, the interaction between the radiation and the substance is measured by the wavelength or frequency of the radiation, resulting in the generation of a spectroscopic signal. The spectra data are commonly obtained by X-ray diffraction (XRD) spectra and Raman spectra. XRD spectra, represented as plots of X-ray intensity versus the angle between the incident and diffracted beams, provide quantitative information about crystal structures, such as the positions and intensities of diffraction peaks, which correspond to interplanar spacings and crystallite sizes. Raman spectra, obtained by measuring the frequency shift of scattered light, provide characteristic information about molecular vibrations and crystal structures. Raman spectra can identify the chemical composition and crystal structure of materials. By delving into spectra data, scientists can gain insight into the composition, structure, and dynamic properties of materials, offering a nuanced understanding of their fundamental characteristics. 

% Through the exploration of spectroscopy, scientists can acquire an understanding of the composition, structure, and dynamic characteristics of materials. 


Chen et al.~\cite{chen2021direct} used a Euclidean neural network (E(3)NN) to predict the phonon density of state (DOS) spectra from atom positions and element types. The E(3)NN model captures symmetries of the crystal structures, with no need to perform data augmentation to achieve target invariances. Hence the E(3)NN model is extremely data-efficient and can give reliable DOS spectra prediction and heat capacity using relatively sparse data of 1200 calculation results on 65 elements. A similar idea was also used to predict the XAS spectra. Carbone et al.\cite{carbone2020machine} used a message passing neural network (MPNN) to predict the O and N K-edge XANES spectra from the molecular structures in the QM9 database7. The training XANES data were generated using the FEFF package. The trained MPNN model reproduced all prominent peaks in the predicted XANES, and 90\% of the predicted peaks are within 1eV of the FEFF calculations. Similarly, Rankine et al.\cite{rankine2020deep} started from the two-body radial distribution function (RDC) and used a deep neural network model to predict the Fe K-edge XANES spectra for arbitrary local environments.


Park~\cite{park2017classification} calculated 150,000 XRD patterns from the Inorganic Crystal Structure Database (ICSD) database and then used CNN models to predict structural information from the simulated XRD patterns. The accuracies of the CNN models reached 81.14\%, 83.83\%, and 94.99\% for space-group, extinction-group, and crystal-system classifications, respectively. Kaundinya~\cite{kaundinya2022prediction} used Atomistic Line Graph Neural Network (ALIGNN) to predict DOS for 56,000 materials in the JARVIS-DFT database using a direct discretized spectrum (D-ALIGNN), and a compressed low-dimensional representation using an autoencoder (AE-ALIGNN). Stein et al.~\cite{stein2019synthesis} tried to learn the mapping between the image and the UV-vis spectrum of the material using the conditional variational encoder (cVAE) with neural network models as the backbone. Such models can generate the UV-vis spectrum directly from a simple material image, offering much faster material characterizations. Predicting gas adsorption isotherms for direct air capture (DAC) are also an important application of spectra-based DL models. 


\subsection{Force Field Development}

% \cite{han2022geometrically}

Force fields or interatomic potentials are sets of potential energy functions and parameters used in atomistic simulations to describe the interactions between atoms within a material. These force fields form the foundation for computational materials design. By learning accurate force fields, researchers can precisely model the behavior of materials at the atomic scale. This leads to a better understanding of the fundamental property-structure relationships in materials, which is crucial for the design of new materials with desired characteristics.


% The force field is a set of potential energy functions and parameters used in atomistic simulations to describe the interactions between atoms within a molecule, setting the bedrock of materials design, including structural optimization, performance prediction, etc. By learning accurate force fields, researchers can precisely model the behavior of materials at the atomic scale, leading to a better understanding of the property-structure relationship.

% Classical force fields typically treat the charge as a fixed atomic property pre-assigned to every atom. In contrast, modern advancements in polarizable force fields, such as the electronegativity equalization method, chemical potential equalization, and charge equilibration, allow for the dynamical adjustment of atomic partial charge. These empirical approaches facilitate the representation of charge evolution through the redistribution of partial charge. Nevertheless, these methods often fall short of accurately capturing the intricacies of complex electron interactions.

% Classical force fields treat the charge as an atomic property that is assigned to every atom a priori. Methodology developments in the field of polarizable force fields such as the electronegativity equalization method, chemical potential equalization and charge equilibration realize charge evolution via the redistribution of atomic partial charge. However, these empirical methods are often not accurate enough to capture complex electron interactions.

Traditionally, there are two diagrams for developing energy functions and parameters, i.e., empirical forcefields and quantum mechanical calculations. Empirical forcefields often rely on hand-crafted parameters, which are efficient yet inaccurate. On the other hand, the estimation of energy functions and parameters can be obtained by extensive optimization to fit the data from quantum mechanical calculations. They are accurate but inefficient. To strike a balance between accuracy and efficiency, machine learning-based methods harness data from quantum mechanical calculations and experiments to identify nonlinear relationships between atomic systems and their forces, offering a promising avenue for supplementing conventional modeling techniques.


% two popular diagrams: empirical forcefields and quantum-mechanical calculations.energy functions and parameters
% extensive optimization and fitting to large datasets of experimental data and quantum chemical calculations, such as density functional theory. 
% Empirical forcefields often rely on hand-crafted parameters, which are efficient yet inaccurate, while ab initio molecular dynamics rely on quantum-mechanical calculations, which are precise but inefficient.


% In contrast, machine learning approaches can harness carefully crafted benchmark data from quantum mechanics-based materials simulations to identify nonlinear relationships between atomic systems and potential energies (or forces). These deep learning-based force fields have facilitated the creation of interatomic potentials that outperform conventional methods in terms of computational cost, accuracy, and versatility, offering a promising avenue for supplementing conventional modeling techniques.

% Molecular dynamics simulation has become an essential tool to understand the microscopic dynamical behaviors of molecular systems. It is worth noting there is a common trade-off between two popular diagrams, empirical forcefields and ab initio molecular dynamics. Empirical forcefields often rely on hand-crafted parameters, which are efficient yet inaccurate, while ab initio molecular dynamics rely on quantum-mechanical calculations, which are precise but inefficient. Inspired by recent advances in deep learning in automated parameters learning and transferability, a large amount of work has been developed to learn machine learning forcefields from quantum-mechanical data to strike a balance between accuracy and efficiency.


% Typically, the energy functions and parameters are obtained by optimizing and fitting through a large amount of experimental data and quantum chemical calculations (e.g., density functional theory). Though these calculations offer the capability to accurately model, such methods remain computationally very demanding. By using carefully created benchmark data from quantum mechanics-based materials simulations, nonlinear relationships between atomic systems and potential energies (or forces more pertinent to the present contribution) could be learned by deep learning. The deep learning-based force field has led to viable pathways for the creation of interatomic potentials that surpass conventional methods both in cost, accuracy, and versatility. 

% In GNN-IPs, atomic structures are represented by collections of nodes and edges, where nodes in the graph correspond to individual atoms and edges are typically defined by simply connecting every atom to all other atoms that are closer than some cutoff distance rc. Every node/atom i is associated with a feature, consisting of scalar values, which is iteratively refined via a series of convolutions over neighboring atoms j based on both the distance to neighboring atoms rij and their features hj. This iterative process allows information to be propagated along the atomic graph through a series of convolutional layers and can be viewed as a message-passing scheme17. Operating only on interatomic distances allows GNN-IPs to be rotation- and translation-invariant, making both the output as well as features internal to the network invariant to rotations.



The pioneer applications of machine learning for crafting interatomic potentials leveraged descriptor-based frameworks with shallow neural networks or Gaussian Processes~\cite{behler2007generalized,bartok2010gaussian,batzner20223}, engineered to maintain invariance with respect to translation, atom permutation within the same chemical species, and rotation. For example, Behler \textit{et. al.}~\cite{behler2007generalized} proposed the first neural network potential, BPNN. In their formulation, an atomic descriptor (i.e., basis functions that transform an atomic configuration into a fixed-length fingerprint vector) based on the bond lengths and bond angles is passed to an MLP (the multilayer perception). On top of this formulation, a Monte Carlo dropout technique can be applied to the MLP to equip the potential with the ability to quantify its predictive uncertainty. 

Recently, geometric GNNs have emerged as powerful deep-learning paradigms for interatomic potentials due to their superior ability to incorporate invariant/equivariant symmetry constraints and long-range interaction~\cite{deng2023chgnet}. They eliminate the need for hand-crafted descriptors. DimeNet~\cite{gasteigerdirectional} expands on using pairwise interactions in a single convolution to include angular, three-body terms, but individual features are still comprised of scalars (distances and three-body angles are invariant to rotation). Cormorant~\cite{anderson2019cormorant} uses an equivariant neural network for property prediction on small molecules. This method is demonstrated on the potential energies of small molecules but not on atomic forces or systems with periodic boundary conditions. PotNet \cite{lin2023efficient} models interatomic potentials by including the Coulomb potential, London dispersion potential, and Pauli repulsion potential. PotNet employs a message-passing scheme that considers interatomic potentials as well as efficient approximations to capture the complete set of potentials among all atoms. 


% In this part, we summarized recently proposed geometric GNN-based interatomic potentials, including DimeNet, TFN, NequIP, CHGNet, MACE, M3GNet, etc.

% MEGNet

% DimeNet

% %Cormorant uses an equivariant neural network for property prediction on small molecules. 
% Tensor-Field Networks directly predict atomic force vectors. 
% TFN


Despite the progress made, previous methods often require large training sets of quantum mechanics-based calculations. This computationally expensive data collection process has become a bottleneck in developing force fields. To improve the data efficiency, NequIP~\cite{batzner20223} uses relative position vectors instead of simple distances (scalars), which not only contain scalars but also features of high-order geometric tensors. This changes the features to be rotation invariant and allows rotation invariant filters to use angle information. NequIP employs E(3)-equivariant convolutions for interactions of geometric tensors, resulting in state-of-the-art accuracy and excellent data efficiency.



Most previous geometric GNN-based force fields are based on two-atom interactions, known as two-body information, which means they only rely on the states of two atoms, known as two-body interactions. This is clearly not in line with the actual situation. However, multi-body interactions often lead to an increase in computational costs. MACE~\cite{batatia2022mace}, an architecture combining equivariant message passing with the efficient many-body message, can capture four body interactions with only two message passes while balancing accuracy and efficiency.

Previous works were specifically developed on a limited number of crystals, such as Li7P3S11 and LixSiy, for lithium-ion batteries, and they failed to generalize to a wide range of materials from different domains. To mitigate the issue, Chen \textit{et al.} proposed a universal graph deep learning for modeling interatomic potential modeling called M3GNet. M3GNet utilizes the largely untapped dataset of more than 187,000 energies, 16,000,000 forces, and 1,600,000 stresses from structural relaxations performed by the Materials Project to train the graph deep learning model. Moreover, a many-body computation module is devised to calculate the three-body and many-body interaction atom indices and the associated angle. M3GNet showcases the potential to learn the interatomic potential of various materials across the periodic table.

\begin{figure}[!t] 
  \centering   
  \includegraphics[width=6.3in]{fig/forcefield.pdf}
  \caption{} 
  \label{fig:forcefield}
\end{figure}
%\end{comment}


However, the inclusion of the important effects that valences have on chemical bonding remains a challenge for neural network potentials, and the early success derived mostly from the inclusion of electrostatics for long-range interaction. The importance of an ion’s valence derives from the fact that it can engage in very different bonding with its environment depending on its electron count. While traditional neural network potentials treat the elemental label as the basic chemical identity, different valence states of transition-metal ions behave differently from each other as different elements. To narrow the research gap, CHGNet~\cite{deng2023chgnet} takes a crystal structure with unknown atomic charges as input and outputs the corresponding energy, forces, stress, and magnetic moments (magmoms). The charge-decorated structure can be inferred from the on-site magmoms and atomic orbital theory. CHGNet regularizes the node-wise features at the convolution layer to contain the information about magmoms. The regularized features carry rich information about both local ionic environments and charge distribution. Therefore, the atom features used to predict energy, force, and stress are charge constrained by their charge-state information. As a result, CHGNet can provide charge-state information using only the nuclear positions and atomic identities as input, allowing the study of charge distribution in atomistic modeling.

% CHGNet~\cite{deng2023chgnet} defines charge as an atomic property (atomic charge) that can be inferred from the inclusion of magnetic moments (magmoms). We show that by explicitly incorporating the site-specific magmoms as the charge-state constraints into the Crystal Hamiltonian Graph Neural Network (CHGNet), one can both enhance the latent-space regularization and accurately capture electron interactions. 
% The foundation of CHGNet is a GNN, where the graph convolution layer is used to propagate atomic information via a set of nodes connected by edges. 

% https://cloud.tencent.com/developer/article/2248677
%https://blog.csdn.net/frank_haha/article/details/132516136

The generalizability of the neural network potentials relies heavily on the amount of labeled training data obtained by DFT. To reduce the cost of DFT labeled samples, Shui \textit{et al.} \cite{shui2022injecting} proposes two strategies to achieve weakly supervised learning of neural network potentials by utilizing physical information in empirical force fields. The first strategy is to train a classifier to select the best possible empirical force field for unlabeled samples and use the energy value calculated from this force field as the label value for the unlabeled sample to achieve data augmentation. The second strategy is based on transfer learning, which first trains on a large dataset obtained through empirical force fields and then uses DFT-labeled samples for fine-tuning. The experiment shows that the first strategy can improve performance by 5\% -51\%, while the second strategy can improve performance by up to 55\%.

% These descriptor-based machine-learning interatomic potentials, exemplified by ænet and DeepMD, have demonstrated encouraging results in bridging the productivity gap between resource-intensive electronic structure methods and efficient classical interatomic potentials.



% The first applications of machine learning for the development of interatomic potentials were built on descriptor-based approaches combined with shallow neural networks or Gaussian Processes, designed to exhibit invariance with respect to translation, permutation of atoms of the same chemical species, and rotation. Machine-learning interatomic potentials such as AENET and DeepMD have provided promising solutions to bridge the gap between expensive electronic structure methods and efficient classical interatomic potentials~\cite{deng2023chgnet}.


% Due to the superior ability to model structural information, graph deep learning models have been shown to yield highly accurate predictions of energies and/or forces of molecules and crystals. Specifically, graph neural network (GNN)-based interatomic potential such as DimeNet, NequIP, TeaNet and MACE have been shown to achieve state-of-the-art performance by incorporating invariant/equivariant symmetry constraints and long-range interaction through graph convolution~\cite{deng2023chgnet}. 
% Recently, geometric GNNs invariant graph neural network interatomic potentials have emerged as a powerful architecture for deep learning of interatomic potentials


% GNN-IPs eliminate the need for hand-crafted descriptors and allow us to instead learn representations on graphs of atoms from invariant features of geometric data (e.g., radial distances or angles). A series of related methods have also been proposed: DimeNet expands on using pairwise interactions in a single convolution to include angular, three-body terms. Cormorant uses an equivariant neural network for property prediction on small molecules. Tensor-Field Networks directly predict atomic force vectors. 





% Most recently, GNN-based MLIPs trained on the periodic table (for example, M3GNet) have demonstrated the possibility of universal interatomic potentials that may not require chemistry-specific training for each new application18,19,20.

Gao \textit{et al.}~\cite{gao2022supervised} pre-trained the neural network potential on a dataset with 86 million molecules. Experiments have shown that compared to training from scratch, the pre-trained network fine-tuning model has significantly improved performance in 7 molecular prediction property tasks and 5 force field tasks. The author also proposes a linear detection approach, which verifies that this strategy can effectively predict many molecular properties, including atomic type, interatomic distance, and molecular skeleton type, by analyzing the molecular representations learned in the pre-training process of the network layer-by-layer.

% Molecular dynamics simulations are widely used in various fields of natural science. Machine learning force fields are replacing ab initio first-principles methods to directly predict forces from the atomic structure of molecules. Due to its advantages of balancing computational speed and accuracy, it is expected to reproduce real molecular dynamics trajectories. However, the current evaluation criteria for machine learning force fields are limited to the prediction accuracy of force and energy, which is far from sufficient for the above objectives. 
% Fu \textit{et al.}~\cite{fu2023forces} selected a series of systems, including water, organic small molecules, peptides, and crystal materials, and designed a series of evaluation criteria to describe trajectory stability, demonstrating that some machine learning force fields with high accuracy currently cannot reproduce dynamics trajectories well. Fu \textit{et al.}~\cite{fu2023forces} proposes that stability should become a new criterion for evaluating machine learning force fields.



% Materials modeling approaches largely fall in two broad categories: one based on quantum mechanical methods , and the other based on interatomic potentials or force fields.
% Quantum mechanical methods (also referred to as ab initio or first-principles methods) are versatile and offer the capability to accurately model a range of chemistries and chemical environments. However, such methods remain computationally very demanding.




% \subsection{Atomistic Image Classification}


% Materials researchers have developed a broad portfolio of applications of computer vision for accelerating and improving image-based material characterization techniques. The images obtained by microscopy techniques range from capturing local atomic to mesoscale structures (microstructure), the distribution and type of defects, and their dynamics which are critically linked to the functionality and performance of the materials. 


% \subsection{Chemical Natural Language Processing}
% \subsection{Conduct Review Based on Data Representation}


\section{Benchmarking and Software Platforms}


\begin{table*}[htbp]\small
  \centering
  \caption{Summary of Common Dataset}
  %  \rowcolors{2}{gray!25}{white}
      \rowcolors{2}{gray!25}{white}
\renewcommand\arraystretch{1.35}
\scalebox{0.83}{
    \begin{tabular}{llll}
    \toprule
    Dataset & Specific Type & URL\\
    \midrule
     Materials Project  (MP)~\cite{jain2013commentary} & -  & \url{https://next-gen.materialsproject.org/}\\
     
     JARVIS-DFT~\cite{choudhary2020joint} & -  &  \url{https://jarvis.nist.gov/}\\
     
    OQMD~\cite{saal2013materials,kirklin2015open} & -   & \url{http:/oqmd.org}\\

Perov-5~\cite{castelli2012new} & Perovskite materials structure &\url{https://github.com/txie-93/cdvae/tree/main/data/perov_5}\\

Carbon-24~\cite{carbon2020data} & Carbon materials structure  &\url{https://figshare.com/articles/dataset/Carbon24/22705192}\\

%Phonon DOS dataset~\cite{chen2021direct} & phonon density of states data for materials  &  103 &\url{https://github.com/zhantaochen/phonondos_e3nn}\\

Crystallography Open
Database (COD)~\cite{vaitkus2021validation} & -  &\url{https://www.crystallography.net/}\\

Raman Open
Database (ROD)~\cite{el2019raman} & Raman spectra&\url{https://solsa.crystallography.net/rod/index.php}\\

The Open Catalyst Project~\cite{zitnick2020introduction} & Catalysts &\url{https://opencatalystproject.org/}\\

MatBench~\cite{dunn2020benchmarking} & Toolkit for materials &\url{https://github.com/materialsproject/matbench}\\

$M^{2}$ Hub~\cite{du2023m} & Toolkit for materials &\url{https://github.com/yuanqidu/M2Hub}\\

Phonon DOS dataset~\cite{petretto2018high} & Phonon density of states &\url{ https://doi.org/10.6084/m9.figshare.c.3938023}\\

    \bottomrule
    \end{tabular}%
    }
  \label{tab:generation}%
\end{table*}%


% \subsection{Datasets}
In addition to various advanced models, datasets and metrics are crucial for AI research in crystallography. A sufficient amount of data helps models better capture the underlying data distribution. Different AI for crystal tasks also rely on corresponding datasets, while appropriate metrics are key for evaluating and optimizing these models. Here, we  introduce common datasets in crystal research and some metrics used for algorithm evaluation.

\begin{enumerate}


\item \textit{The Materials Project }~\cite{jain2013commentary}:
The Materials Project (MP) is a scientific initiative that offers open access to a comprehensive database of computed properties of materials, aimed at accelerating innovation in materials. Initiated in 2011, the project leverages the capabilities of supercomputers along with cutting-edge quantum mechanics theories and density functional theory (DFT) to systematically compute the properties of thousands of materials. 
Currently, the MP dataset includes over 120K materials with the complete specification of their crystal structure and some important physical properties like band gap, energy above hull and so on.

\item \textit{JARVIS-DFT}~\cite{choudhary2020joint}:
The joint automated repository for various integrated
simulations (JARVIS) provides a large-scale computational dataset containing thousands of crystalline materials. 
As part of JARVIS, JARVIS-DFT was launched in 2017 and contains data
for approximately 40,000 materials, with about 1 million calculated properties, such as the crystal's space group, bandgaps, and Bulk Moduli. 


\item \textit{OQMD}~\cite{saal2013materials,kirklin2015open}:
The open quantum materials database (OQMD) is a database of thermodynamic and structural properties of inorganic materials based on high-throughput DFT calculations, currently containing over 800,000 crystal structures. In addition to crystal structure generation and crystal material performance prediction, it has also been applied to various other types of material problems \cite{saal2013materials}.

\item \textit{Perov-5}~\cite{castelli2012new}:
Perov-5 is a dataset tailored for research on perovskite crystalline materials, comprising 18,928 different perovskite materials. All materials possess the similar perovskite crystal structure but vary in composition. Moreover, the dataset includes 56 elements, and the unit cell within all materials contains five atoms.

\item \textit{Carbon-24}~\cite{carbon2020data}:
Carbon-24 is a specialized scientific dataset for carbon materials, containing over 10,000 different carbon material structures that have the same composition but different structures. Each material consists of one element, with 6 to 24 atoms within the unit cell. Additionally, Carbon-24 provides comprehensive data on the physical, chemical, and mechanical properties of each material, including electronic performance, thermal stability, and mechanical strength.


\item  \textit{Crystallography Open
Database}~\cite{vaitkus2021validation}: 
The Crystallography Open Database (COD) is a crystallography database that specializes in collecting and storing crystal structure information for inorganic compounds, small organic molecules, metal-organic compounds, and minerals. It includes specific details such as crystal structure parameters (unit cell parameters, cell volume, etc.), space group information, and allows for the export of crystal information files in CIF format.

\item \textit{Raman Open
Database }~\cite{el2019raman}: The Raman Open Database (ROD) is an open database that specializes in collecting and storing Raman spectroscopy data. It contains a large amount of Raman spectral data for crystalline materials, including the chemical formulas of the materials and corresponding Raman spectral information such as excitation wavelengths and intensities.

\item \textit{The Open Catalyst Project}~\cite{zitnick2020introduction}:
The goal of the Open Catalyst Project is to utilize artificial intelligence to simulate and discover new catalysts for renewable energy storage, aiming to help combat climate change. Currently, the Open Catalyst Project includes datasets such as Open Catalyst 2020 (OC20) and Open Catalyst 2022 (OC22), which are used to train machine learning models. These datasets collectively contain 1.3 million DFT structural relaxations (the structure in which the atomic positions have been
optimized to find the configuration with the lowest energy) and results from over 260 million single point evaluations. They cover a wide range of crystal surfaces, and adsorbates (molecules containing nitrogen, carbon, and oxygen chemistries). Besides, these datasets are divided into training, validation, and test sets, representing common situations in catalysis: predicting the properties of a previously unseen adsorbate, for a previously unseen crystal structure or composition, or both.


\item \textit{MatBench}~\cite{dunn2020benchmarking}: MatBench is a benchmark test suite in the field of materials science, which can be used to evaluate and compare the performance of various machine learning models in predicting material properties. The original datasets used in MatBench primarily come from multiple public databases in materials science, such as OQMD, MP, etc. Additional modifications are then enumerated to tailor the datasets for machine learning applications.


\item \textit{$M^{2}$ Hub}~\cite{du2023m}: $M^{2}$ Hub is a machine learning toolkit for materials discovery research that covers the entire workflow, including problem formulation, data downloading, data processing, machine learning method implementation, machine learning training and evaluation procedures, as well as benchmark results and evaluations. In terms of datasets, $M^{2}$ Hub includes 9 public datasets, such as MP and Carbon24, covering 6 types of materials and involving 56 tasks related to eight material properties.


\item \textit{Phonon DOS dataset}~\cite{petretto2018high}: 
Phonon DOS dataset contains approximately 1,500 crystalline materials whose phonon DOS is calculated
from density functional perturbation theory (DFPT). 
Most materials in the dataset have less than 13 atomic sites per cell.

\end{enumerate}

%Besides the common datasets mentioned above, there are also some benchmarks developed based on these datasets, as follows. Phonon DOS dataset\footnote{\url{https://github.com/zhantaochen/phonondos_e3nn}} used in \cite{chen2021direct} contains phonon density of states data for materials that collects from the MP. Is is a small training set of about 1000 samples across more than 64 types of atoms.








% \subsection{Metrics}

% \subsubsection{Metrics for Property prediction}
% The task of property prediction for crystalline materials typically employs supervised methods with real property labels, so performance evaluation in most works uses metrics such as the mean absolute error (MAE) or the root mean squared error (RMSE) \cite{taniai2024crystalformer,wang2024conformal,yan2024complete}.

% Additionally, some more complex evaluation methods have also been studied to a certain extent. 
% Recently,
% Varivoda et al.\cite{varivoda2023materials}
% presented a benchmark study of
% ML models for property prediction with uncertainty quantification.
%  Omee et al. \cite{omee2024structure} propose an OOD (Out-Of-Distribution) materials property prediction benchmark. This benchmark proposes five different approaches to generate OOD test sets for the selected datasets. Using these datasets and the OOD test sets, the performance of GNN models in predicting OOD material properties is evaluated.

% \subsubsection{Metrics for Structure Generation}

% Due to the randomness in material generation, the evaluation metrics for crystal material generation tasks are more diverse than those for crystal material performance prediction tasks. Firstly, RMSE is also a common metric in generation tasks, typically used to measure the error between the true value and the best matching candidate. Additionally, since the lattice volumes of different materials are inconsistent, the RMSE values need to be normalized by $\sqrt[3]{V/N}$, where $V$ is the lattice volume and $N$ is the number of atoms in the lattice.

% The match rate is another common metric for evaluating the quality of generated crystal structures. It is used to compare the similarity between the generated structures and known or target structures, typically measured as the ratio of the number of generated structures that match the total number in the test set.

% In addition to the direct calculation of match rate and RMSE to evaluate the quality of generated structures, 
% some works also use other metrics to assess the generation performance.
% \cite{gruver2024finetuned} use stability metrics like ML potential \cite{chen2022universal}.
% If the calculated energy above hull is higher than 0.1 eV/atom, the generated material can be considered unstable.
% In \cite{xie2021crystal},
% structural validity depends on whether the shortest distance between any pair of atoms is greater than $\text{0.5 Å}$, while compositional validity
% captures the net charge of the structure (The composition is valid if the overall charge is neutral). 
% \cite{gruver2024finetuned} also evaluate the diversity of generated structures by generating the CrystalNN fingerprints \cite{zimmermann2020local} for each structure. They calculate the L2-distances between all pairs among 20 samples of each composition, using the mean and maximum of these distances as evaluation metrics.






\section{Insights and Future Outlooks}

\subsection{Explainability}

Though the uptake of deep learning for materials science is at an exciting, early stage, to realize the true potential of machine learning models for successful scientific discovery, they must have qualities beyond purely predictive power. The predictions and inner workings of models should provide a certain degree of explainability by human experts, permitting the identification of potential model issues or limitations, building trust in model predictions, and unveiling unexpected correlations that may lead to scientific insights. In this paper, we have outlined observations of the nascent field of explainable methods in the context of materials science and provide insights into potential future research directions.

Recently, many explainable machine-learning methods have been proposed to tackle the issue of limited interpretability to enhance human cognition and decision-making capabilities. For the purpose of interpretability~\cite{Selvaraju_2017_ICCV,fel2023don,agarwal2021towards,vu2020pgm,huang2022graphlime}, existing explainable machine-learning methods can be generally classified into two classes: post-hoc methods to explain black-box models and intrinsic methods to create white-box models~\cite{turbe2023evaluation,linardatos2020explainable}. Post-hoc interpretability refers to how a trained model makes predictions and uses the input features it is given, whereas intrinsic interpretability aims to study how to use transparent individual constituents to construct a model. 

Currently, several post-hoc interpretability techniques have been employed in materials science. Some Transformer-based prediction methods utilize attention weights as explanations, and the intuition of these methods is that important features will have higher attention weights. For example, Uni-MOF~\cite{wang2024comprehensive} pre-trained a Transformer-based for gas adsorption predictions in metal-organic frameworks. Since the multi-head attention mechanism of the Transformer can learn the interactions within the material structure, Uni-MOF derives attention maps of atoms to depict the interactions between the metal sites. Uni-MOF finds chemically linked atoms have a larger attention value, thus confirming the reliability of predictions. SCANN~\cite{vu2023towards} incorporates the attention mechanism to predict material structure properties and provide meaningful information about the structure-property relationships, where attention scores are used to indicate the importance of each local structure contributing to the accurate prediction. However, recent studies suggest that "attention is not explanation" because attention weights are often inconsistent with the feature importance~\cite{serrano2019attention}. 

Instead of using attention, CrysXPP~\cite{das2022crysxpp} uses trainable weights w.r.t features to indicate the feature importance. CrysXPP introduces a feature selector that helps to provide an explanation by highlighting the subset of the atomic features responsible for the manifestation of a chemical property of the given crystal. The node features are first passed through a feature selector, which is a trainable weight vector that selects a weighted subset of important node-level features for a given property of interest. With case studies in material, CrysXPP shows that the feature selection module can effectively provide explanations of the importance of different features towards prediction, which are in sync with the domain knowledge. 


% CrysXPP~\cite{das2022crysxpp} proposes an explainable deep property predictor based on the auto-encoder-based architecture.


% such as features-based methods~\cite{Selvaraju_2017_ICCV} and perturbation-based methods~\cite{fel2023don,agarwal2021towards} 

% These methods can be categorized into four classes: gradients/, such as Grad-CAM, surrogate-based methods~\cite{vu2020pgm,huang2022graphlime}, and .

Perturbation-based methods perturb the inputs and evaluate the output changes to reveal the relationship between the input and output~\cite{fel2023don,agarwal2021towards}. The intuition of this type of method is that perturbing important feature pairs will have a significant impact on model predictions. CGCNN~\cite{xie2018crystal} learns the contribution of different local chemical environments, represented by the scalar for each atom, to the target property. The interpretability is demonstrated by learning the energy of each site in perovskites from the total energy above hull data. Perovskite is a crystal structure type with the form of ABX3, where the site A atom sits at a corner position, the site B atom sits at a body-centered position, and site X atoms sit at face-centered positions. The authors observe that elements with small radii like Be, B, and Si are the most unstable elements for occupying the A site. For the B site, elements in groups 4, 5, and 6 are the most stable throughout the periodic table. This can be explained by crystal field theory since the configuration of d electrons of these elements favors the octahedral coordination in the B site. This provides additional insights for material design. However, some studies suggested that generated explanations may change drastically with very small perturbations, and the generated explanations are not robust~\cite{agarwal2021towards}. 

% CGCNN~\cite{xie2018crystal} maps the last atom feature vector to a scalar and performs a linear pooling to predict the target property directly. In particular, 

Interpretability methods of white-box models encompass methods that create interpretable and easily understandable models. The models in this category are often called intrinsic, transparent, or white-box models. Such models include the linear, decision tree, and rule-based models. To unravel the correlation between adsorption energy and the properties of the adsorbate-catalyst system, Vinchurkar \textit{et. al.}~\cite{vinchurkar2024explainable} used SHapley Additive exPlanations (SHAP) analysis~\cite{lundberg2017unified} to provide the top five importance features: adsorbate electronegativity, the number of adsorbate atoms, catalyst electronegativity, effective coordination number, and the sum of atomic numbers of the adsorbate molecule. Based on the features, the rule-based method --- symbolic regression~\cite{wang2019symbolic,makke2024interpretable} derives mathematical equations to compute the adsorption energy. These equations are compared to equations obtained from traditional theory or experimental-based methods, providing complementarity insights into the relation of adsorption energy with structural properties. Similarly, Anker \textit{et. al.} ~\cite{anker2022extracting} applied gradient boosting decision trees to predict Rwp values to quantify how important each atom or feature in the structure is.

Although these pioneering works have explored interpretability in materials science, many challenges remain unresolved. 1) Limited explainability scale: Due to complex and non-linear relationships between material properties and features, material properties can depend on features at different scales, including atomic, microstructural, and macroscopic. The existing methods can only explore the correlation between structure and properties from microscopic and single-scale features, limiting a deeper understanding of the relationship between structure and properties. 2) Interdisciplinary knowledge requirement: Understanding materials science requires knowledge of physics and chemistry, making it challenging to create interpretable models that are accessible to all researchers from different fields. Moreover, incorporating domain-specific knowledge into models can be challenging in machine-learning contexts. Therefore, relevant benchmarks and ground truth are needed in the field of materials science to promote the development of interpretable models in this interdisciplinary. 3) Trade-off between explainability and model performance: Deep learning models provide exceptional performance, however, deep learning models are typically considered "black boxes" due to their complex, multi-layered architectures and the non-linear transformations of input data. This makes it challenging to understand the internal decision-making process and explain the model's outputs. White box models are generally less complex and more interpretable than deep learning models. However, they may not achieve comparable performance, especially on complex, non-linear problems. 4) Explainability robustness: although there are numerous interpretable methods available, such as attention-based, gradient-based, perturbation-based, etc., they may not necessarily produce robust and faithful explanations~\cite{agarwal2021towards,wang2024explainable,rudin2019stop,serrano2019attention}. In particular, experimental data often contains noise from measurement uncertainties and environmental conditions, which may be harmful to the robustness and faithfulness of obtained explanations.



% Gradient-based methods determine the feature importance by the partial derivatives of the output to each feature~\cite{Selvaraju_2017_ICCV}. However, several works show that the gradient-based methods may not be reliable, as they disregard the influence of model architectures on the output and fail to incorporate the information of the model architectures into the explanations~\cite{agarwal2021towards,rudin2019stop}.


% The authors demonstrated the interpretability by learning the energy of each site in perovskites from the total energy above hull data. 

% To unravel the correlation between adsorption energy and the properties of the adsorbate-catalyst system, Vinchurkar \textit{et. al.}~\cite{vinchurkar2024explainable} employed two techniques, posthoc XAI analysis and symbolic regression, .
% The post-hoc analysis uses shallow regression models like XGBoost for predicting adsorption energy and use 




\subsection{Self-Driving Laboratories}


Material discovery processes involve sequentially screening a large pool of candidates. This step, known as sequential experimentation, aims to identify target material with desired properties. Self-driving or autonomous laboratories~\cite{burger2020mobile,pyzer2022accelerating} use machine learning models to plan and perform experiments, increase the level of laboratory automation, and show the potential to accelerate the material discovery processes. Currently, self-driving laboratories have offered the promise of small molecule discovery. However, the research on material science is very limited. In this section, we first highlighted representative works on self-driving laboratories and provided some clues for self-driving laboratories on material science.


In these years, self-driving laboratories have covered the automation of retrosynthesis analysis (such as in reinforcement-learning-aided synthesis planning~\cite{segler2018planning,coley2019robotic}), prediction of reaction products (such as in CNNs for reaction prediction~\cite{coley2019graph}) and reaction condition optimization (such as in robotic workflows optimized by active learning~\cite{granda2018controlling,burger2020mobile}). However, the scarcity of training data presents challenges such as instability and susceptibility to overfitting when training these models from scratch. In recent years, the rise of large-scale models has brought new insights into self-driving laboratories. Fueled by ever-expanding textual datasets and significant increases in computing power, LLM-based agents are capable of chain-of-thought reasoning, self-reflection, and decision-making. These autonomous agents are typically augmented with tools or action modules, empowering them to go beyond conventional text processing and directly interact with the physical world, e.g., scientific experimentation~\cite{miret2024llms,m2024augmenting,jia2024llmatdesign}. One recent representative work is ChemCrow~\cite{m2024augmenting}. By combining the reasoning power of LLMs with chemical expert knowledge from 18 computational tools in chemistry, ChemCrow showcases one of the first chemistry-related LLM agent interactions with the physical world. ChemCrow has successfully planned and synthesized an insect repellent and three organocatalysts and guided the screening and synthesis of a chromophore with target properties. Jia \textit{et. al.} introduced LLMatDesign, a LLM-based framework for materials design. LLMatDesign~\cite{jia2024llmatdesign} utilizes LLM agents to translate human instructions, apply modifications to materials, and evaluate outcomes using provided tools. By incorporating self-reflection on its previous decisions, LLMatDesign adapts rapidly to new tasks and conditions in a zero-shot manner. An evaluation of LLMatDesign on several materials design tasks, in silico, validates LLMatDesign's effectiveness in developing new materials with user-defined target properties in the small data regime. 

Despite successful proof-of-concept examples of self-driving laboratories in the accelerated synthesis of molecules and materials, many opportunities exist for further research and development. 

1) Human–AI collaboration: While AI technologies excel at handling large datasets, pattern recognition, and the execution of repetitive experimental protocols, they lack the depth of understanding, creativity, and contextual awareness that human researchers bring.  First, humans must validate AI's operations, ensuring they align with accepted scientific principles, safety, and ethical standards. This dual involvement helps mitigate risks associated with erroneous interpretations and maintains research integrity. Second, experiments often lead to unexpected results that require immediate rethinking and adjustments to protocols. In these scenarios, human judgment is invaluable~\cite{liu2023conversational}. By actively involving human experts in the research loop, their knowledge can be leveraged to inform the selection of relevant materials, the design of experiments, and the interpretation of findings~\cite{liu2022machine,tiihonen2022more,SUN20211305}. For example, Bayesian optimization can be combined with automation to form semi- or fully autonomous materials optimization loops in self-driving materials laboratories, in which an acquisition function can incorporate domain knowledge and human experts as probabilistic constraints for guiding the discovery~\cite{liu2022machine}. In this aspect, large language models could play a significant role in enhancing the "humans in the Loop" approach due to the conversational interface, which enables users to incorporate feedback, design concepts, and prior knowledge into the LLMs. 


2) Configurable module integration: The adoption of self-driving laboratories by scientists across chemical and materials sciences would entail highly intelligent and flexible automation of research labs with autonomously reconfigurable experimental modules~\cite{abolhasani2023rise}. An important software aspect of self-driving laboratories is their flexible integration with machine learning to provide autonomy for navigation through the design space of molecules and materials. The rapidly growing list of machine learning modeling and experiment selection strategies makes algorithm selection a challenging task for non-experts. This challenge is an exciting opportunity for the future development of self-driving laboratories toward the standardization of machine learning algorithms suitable for different end-to-end experimental workflows and operation modes (exploration, exploitation, or mechanistic studies).

3) Material language processing: The challenge of the autonomous development for materials, in contrast to that of small molecules, is the lack of data related to material language processing. Materials language processing can facilitate materials science research by automating the extraction of structured data from research papers. Despite the existence of deep learning models for materials language processing tasks, there are ongoing practical issues associated with complex model architectures, extensive fine-tuning, and substantial human-labeled datasets. Choi \textit{et. al.} ~\cite{choi2024accelerating} presented a GPT-enabled pipeline for materials language processing tasks, providing guidelines for text classification, named entity recognition, and extractive question answering. However, this method can only handle textual data and cannot capture the geometry of the material. This failure, however, creates a unique opportunity. Researchers can use multimodal large models to capture both textual information and material geometry simultaneously. In addition, retrieval augmented generation can be incorporated into self-driving laboratories to supplement the model output by using external data, ensuring more accurate and up-to-date output to address the low-data issue in material languages~\cite{gao2023retrieval,lewis2020retrieval}.

 
 % To address the challenge, the humans in the discovery process, often referred to as "humans in the loop," can be involved. Material scientists possess deep domain expertise accumulated through years of training and hands-on experience. By actively involving these experts in the research loop, their knowledge can be leveraged to inform the selection of relevant materials, the design of experiments, and the interpretation of findings. However, directly introducing humans would severely slow down the otherwise accelerated optimization loop\cite{tiihonen2022more}. BO can be combined with automation to form semi- or fully autonomous materials optimization loops in self-driving materials laboratories, in which an acquisition function can incorporate with domain knowledge and human experts as probabilistic constraints for guiding the discovery\cite{liu2022machine}. Armi\textit{et. al.} \cite{tiihonen2022more} proposed to add humans into the Bayesian optimization loop to evaluate candidate quality, and query them only when human opinion is needed to prevent the humans from becoming a bottleneck in the loop. Sun et al.\cite{SUN20211305} incorporated density functional theory calculations of phase stability as a probabilistic constraint for the experimental acceleration of composition optimization to improve perovskite stability, avoiding compositions susceptible to phase segregation. 


% Due to the interactive ability, large language models can play a significant role in enhancing the "humans in the Loop" approach for material design and discovery~\cite{liu2023conversational}. Large language models trained on vast amounts of scientific literature can serve as powerful tools for extracting relevant information, identifying key concepts, and synthesizing knowledge from a wide range of material science research. On the other hand, large language models allow for a dynamic exchange of information, enabling users to incorporate feedback from prior knowledge or domain experts into the model by using the conversational interface, and designers can use language models to verbalize or describe their design concepts and receive instant feedback on those ideas. This can help refine designs and identify potential issues early in the process in a conversational way.



\subsection{Generalizability}


 % However, their performance heavily depends on the availability and quality of training data. In cases of insufficient or biased data, these algorithms risk poor performance, leading to ineffective or misleading results. 

Deep learning has demonstrated the potential to accelerate the material discovery process. However, they suffer from generalizability issues in material science, as their performance on new or unseen data could deteriorate. Specifically, the generalizability issues could be reflected in three aspects. First, due to the discovery of new materials, the distribution of new data may shift from the training data distribution of the model, i.e., out-of-distribution~\cite{omee2024structure}. If a model is trained on a specific set of crystal structures but encounters a new, unfamiliar structure during testing or application, it may struggle to provide accurate predictions since it hasn't been exposed to such variations. Second, crystalline materials can exhibit different behaviors under extreme conditions such as high temperature, pressure, or strain~\cite{wang2024comprehensive}. Models trained on data within normal ranges might fail to generalize to these extreme conditions. Third, crystal defects, such as vacancies, interstitials, or dislocations, introduce variations that might not be adequately captured by models trained on defect-free structures, contributing to the generalizability challenge~\cite{ziletti2018insightful}.
In this section, we review some efforts towards generalization and then point out some directions.



% In particular, due to the discovery of new materials, the distribution of new data may shift from the training data distribution of the model, i.e., out-of-distribution. 

% The constantly emerging data requires highly demanding generalizability of models in material science and computational modeling. 



% In crystalline materials research, this can occur due to various reasons: 1) Novel Crystal Structures~\cite{omee2024structure}: If a model is trained on a specific set of crystal structures but encounters a new, unfamiliar structure during testing or application, it may struggle to provide accurate predictions since it hasn't been exposed to such variations. 2) Extreme Conditions~\cite{wang2024comprehensive}: Crystalline materials can exhibit different behaviors under extreme conditions such as high temperature, pressure, or strain. Models trained on data within normal ranges might fail to generalize to these extreme conditions, leading to OOD issues. 



% However, the generalizability of deep learning models remains a formidable challenge, as their performance on new or unseen data can significantly deteriorate. This issue is particularly pronounced in the complex and high-dimensional space of crystal materials, where the diversity of structures and compositions presents unique challenges for model generalization.

% Factors contributing to the generalizability challenge can be summarized as follows. 1) Low data regime:  The availability of experimental and computational data for crystal materials is often limited, especially for rarer or more complex structures with specific properties or under specific conditions. This data scarcity can hinder the ability of deep learning models to learn robust and generalizable representations. 2) Complex structure-property relationships: Crystal materials exhibit a wide range of structural variations, including different unit cell sizes, atomic arrangements, and symmetry groups. Therefore, crystal materials can exhibit a vast array of physical, chemical, and electronic properties, such as conductivity, dielectric behavior, ferroelectricity, and catalytic activity. Developing deep learning models that can capture and generalize across this structural diversity and generalize across this broad spectrum of material properties is a complex task.

There have been some efforts towards generalization. Typically, they use pretraining techniques on large-scale databases to improve the generalizability. Uni-MOF~\cite{wang2024comprehensive} used data with conditions such as temperature, pressure, and different gas molecules for fine-tuning, which makes Uni-MOF generalizability in predicting gas adsorption with different associated gas, temperature, and pressure. However, the method can only generalize to MOF material. M3GNet~\cite{chen2022universal} utilizes the largely untapped dataset of more than 187,000 energies, 16,000,000 forces, and 1,600,000 stresses from structural relaxations performed by the Materials Project to train the graph deep learning model. M3GNet showcases the potential to predict the formation energy, etc, of various materials across the periodic table. Compared to the supervised setting, although such pre-trained models have proven to be more effective in generalizing to various downstream tasks by fine-tuning on a few labeled examples, it is still an open challenge to generalize unseen categories and tasks without such labeled examples or fine-tuning (i.e., the so-called zero-shot setting in machine learning).  


% Unsupervised pretraining on large-scale databases has been proposed~\cite{zeng2022accurate}, with the main advantage being the ability to learn chemical structures without supervised annotation by reconstructing the masked topological or geometric substructures. 




To address the generalizability challenge, researchers can explore several strategies that enhance the capabilities of deep learning models in material science. One promising approach involves leveraging physics-informed neural networks, which integrate domain-specific knowledge and physical constraints directly into the modeling process. By doing so, these networks could capture the underlying principles that govern crystal materials, ultimately paving the way for the development of universal machine-learning models in materials science \cite{azizzadenesheli2024neural}.
Additionally, generating augmented or synthetic data can significantly enrich training datasets and include a broader array of material variations, thus improving model generalization capabilities \cite{ma2020data}. Traditional molecule pretraining methods have predominantly focused on chemical structures, which tends to limit the exploration of multi-modal representations. Recent advancements propose methodologies that model molecules through one-dimensional descriptions, two-dimensional molecular graphs, or three-dimensional geometric structures, addressing various downstream tasks and enabling a more comprehensive understanding of molecular behavior \cite{liu2023multi, fang2024moltc, luo2023molfm}. However, the exploration of multimodal data in the field of materials science is still in its infancy.
Furthermore, employing techniques for uncertainty or confidence estimation is crucial, as it allows researchers to quantify model uncertainty and reduce the likelihood of erroneous predictions. 


\subsection{Unified Benchmarking}

Amidst an influx of emerging work, comparative assessments are often impeded by inconsistencies in datasets, architectures, metrics, and other evaluation factors. To enable healthy progress, there is a pressing need to establish standardized benchmarking protocols across tasks. Unified frameworks for fair performance analysis will consolidate disjoint efforts and clarify model capabilities to distill collective progress. Although various datasets are introduced, Material science datasets can vary widely in terms of size, type, and quality of data. Benchmarking deep learning models on heterogeneous datasets can lead to biased evaluations and hinder the generalizability of the results. 
Fortunately, some platforms have already made attempts to benchmark existing datasets and methods. Geom3D \cite{liu2024symmetry}, a platform for geometric modeling on 3D structures, integrates MatBench and QMOF datasets and several geometry neural networks.

Material science tasks, such as energy prediction, molecular design, and materials discovery, present diverse and complex challenges. Benchmarking across these tasks may require specialized evaluation protocols to capture the nuances of each problem domain. Although there are already some indicators for evaluation, they are often inaccurate, and there is still a long way to go before the true value obtained from DFT. However, DFT validation often requires a large amount of specialized domain knowledge, which hinders the in-depth research of machine learning practitioners. Therefore, more comprehensive and convenient indicators or evaluation methods are urgently needed.


% -based crystal representations utilize spectral data to capture and analyze the characteristics of crystal structures. Common examples include . 




% \section{Main text heading 1}

% Please use headings/subheadings to break up the text. Main headings should be no more than 38 characters, including spaces.

% \subsection{Subheading 1}

% Subheadings should be no more than 39 characters, including spaces. In the final layout, subheadings will be in-line and thus followed by a full stop.

% \subsubsection*{Second-level subheading 1}
% Second-level subheadings should be no more than 70 characters, including spaces.

% \section{Main text heading 2}

% \subsection{Subheading 2}
% \subsubsection*{Second-level subheading 2}
% ...\\
% ...

% \section{Outlook/Future Perspectives}
% The text is often best rounded off with a comment on the implications of the latest work and on future research directions.  This section should be about 800 words long and is an opportunity for authors to give their vision of where the field is heading.

% \section{7 display items [figures, text boxes or tables]}

% Display items should be complementary to the main text and avoid repeating information. Please keep in mind that all display items will need to fit in portrait format. Please cite all display items in the main text. Do any items require copyright permission? If any of the figures have been reproduced or adapted from elsewhere we need you to complete a \href{http://www.nature.com/licenceforms/npg/thirdpartyrights-table.doc}{Third Party Rights Table}, which includes the relevant details (including full reference and figure number) so we can request permission from the publishers to use it.  We do not require the Third Party Rights table to be completed before submission of the first draft.  However, to speed up the process at the author revision step, we recommend that you add the reference numbers to the figure captions.  Please note that we cannot use permissions (to adapt/reproduce figures) that authors have received from publishers. Also, a permission is still required if the author of this Review article is an author of the original manuscript.\\

% \noindent For chemical structures, please see the \href {https://www.nature.com/documents/nr-chemical-structures-guide.pdf}{Nature guide for ChemDraw structures}.\\

% \noindent For information about the artwork process at Nature Reviews journals, please refer to \href{https://www.nature.com/reviews/pdf/artworkguide.pdf}{the guide to authors} for figures and an  \href{http://www.nature.com/reviews/pdf/artworkguidep2.pdf}{example figure}.\\



% \noindent \textbf{Figure captions}\\
% \noindent Please include detailed figure captions that define all symbols and abbreviations used in the figures (e.g. $V$, voltage; $R$, resistance). Readers should understand figures without needing to refer to the text. Figure captions should be included in the manuscript latex document. Figures should be provided separately.\\

% \begin{figure}[ht]
% \centering
% %\includegraphics[width=\linewidth]{fig}
% \caption{\textbf{Title.} a | Text. b | Text. c | Text. d | Text maximum 250 words. Panel a is adapted/reproduced with permission from ref.123, Springer Nature Limited. Panel b is adapted/reproduced with permission from ref.124, Publisher Name.}
% \label{fig}
% \end{figure}



% \begin{table}[ht]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% Particle & Mass & Charge \\
% \hline
%  \multicolumn{3}{|c|}{Charged particles}\\
% \hline
% Electron & $9.10938356(11)\times10^{-31}$ kg & $-1e$ \\
% \hline
% Proton & $1.672621898(21)\times10^{-27}$ kg & $+1e$ \\
% \hline
%  \multicolumn{3}{|c|}{Neutral particles}\\
% \hline
% Neutron & $1.674927471(21)\times10^{-27}$ kg & $0$ \\
% \hline
% \end{tabular}
% \caption{\label{tab}Tables have titles but no captions are allowed. All symbols and acronyms used in a table should be defined in a footnote. Example: Here $e$ is the elementary charge.}
% \end{table}


% \section{References} 

\bibliography{mybib}

% 150–200 references are suggested. All referenced work should be accepted for publication or on recognized Archive databases. References should be given superscript numbers and cited sequentially according to where they appear in the main text, followed by those in the text boxes, figure captions and then tables (i.e. the order they appear in this template).
% Journal abbreviation in italics, volume number in bold. If there are six or more authors for a reference, only the first author should be listed, followed by 'et al.'. Journal name abbreviations are followed by a full stop. Please include full page ranges. \\

% \noindent Please do not cite web sites in the reference list — these should be listed separately, with the URLs in the Related Links section (see below).  If you are unsure if the website is a ‘Related link’ or should go in the ‘References’ section then identify if there is a publication date on the website.  If there is a publication date, it is likely that the item will be in the ‘References’ section.  If there is no publication date, it is likely that the item will be in the ‘Related Links’ section.\\

% \noindent When citing a book, please indicate if you are citing a specific page range or chapter.  Otherwise, we presume that you are citing the entire book.  \\

% \noindent \textbf{Highlighted references (optional)} Please select 5–-10 key references and provide a single sentence for each, highlighting the significance of the work.\\

% \noindent\textbf{Acknowledgements}\\
% E.g. Funding agencies.\\

% \noindent\textbf{Author contributions}\\
% Please describe the contributions made by each author.  Please use the initials of the individual author to explain these contributions.  These contributions are also required when you upload the files to our submission website.\\

% \noindent\textbf{Competing interests}\\
% Nature Journals require authors to declare any competing interests in relation to the work described. Information on this policy is available \href{http://www.nature.com/authors/policies/competing.html}{here}. \\



% \noindent\textbf{Supplementary information (optional)}
% If your article requires supplementary information, please include these files for peer-review. Please note that supplementary information will not be edited.


\end{document}
